Mesoscale asymptotic approximations to solutions of mixed boundary value problems in perforated domains

We describe a method of asymptotic approximations to solutions of mixed boundary value problems for the Laplacian in a three-dimensional domain with many perforations of arbitrary shape, with the Neumann boundary conditions being prescribed on the surfaces of small voids. The only assumption made on the geometry is that the diameter of a void is assumed to be smaller compared to the distance to the nearest neighbour. The asymptotic approximation, obtained here, involves a linear combination of dipole fields constructed for individual voids, with the coefficients, which are determined by solving a linear algebraic system. We prove the solvability of this system and derive an estimate for its solution. The energy estimate is obtained for the remainder term of the asymptotic approximation.

==> Mesoscale pdf/Introduction_Meso.tex <==
\begin{abstract}
We describe a  method of  
asymptotic approximations to solutions of  mixed boundary value problems for the Laplacian in a 
three-dimensional domain with many perforations of arbitrary shape, with the Neumann boundary conditions being prescribed on the surfaces of small voids.
%Periodicity of the array of voids is not required, but
The only assumption made on the geometry is that  
the diameter of a void is assumed to be smaller compared to the distance to the  
nearest neighbour. 
%We use the method of mesoscale asymptotic approximations established in the  earlier paper \cite{MMMeso}. 
The asymptotic approximation,
obtained here, involves a linear combination of dipole fields constructed for individual voids, with the coefficients, which are determined by solving a linear algebraic system.
We prove the solvability of this system and derive an estimate for its solution. The energy estimate is obtained for the remainder term of the asymptotic approximation.
%The asymptotic approximation of the solution to a mixed boundary value problem in a body with many small cavities is presented. We do not require any periodicity of the array of holes. The approximation is shown to be constructed from a linear combination of model solutions associated the domain with no perforations and the  exterior of the individual voids, where the coefficients involved are the solution of a linear algebraic system. Invertibility of this system is proved under weak geometrical constraints.  The energy estimate for the remainder given by the approximation is also justified
\end{abstract}
\section{Introduction}\label{Introductionmeso}


In the present paper we discuss a method for  asymptotic approximations to solutions of  the mixed problems for the Poisson equation for  domains  containing  a number, possibly large,  of  %many 
small perforations of arbitrary shape. The Dirichlet condition is set on the exterior boundary of the perforated body, and the Neumann conditions are specified  on the boundaries of small holes. 
%No periodicity constraints are imposed on the position of holes, and 
Neither periodicity nor even local ``almost'' periodicity constraints  are imposed on the position of holes,  which makes the homogenization methodologies not applicable (cf.  Chapter 4 in \cite{MKh}, and Chapter 5 in \cite{SP}).  
Two geometrical parameters, $\varepsilon$ and $d$, are 
introduced to characterize the maximum diameter of perforations within the array and the minimum distance between the voids, respectively. Subject to %a %weak 
the 
%only 
{\em mesoscale} constraint, $\varepsilon < \mbox{const} ~d$, the %mesoscale 
asymptotic approximation to the solution of the mixed boundary value problem is constructed. 
The approximate  %approximation 
solution involves a linear combination of dipole fields constructed for individual voids, with the coefficients
 %, which are 
 determined %by solving 
 from a %model 
 linear algebraic system. 
The formal asymptotic 
representation  is accompanied by the energy estimate of the remainder term.
% for the case when the number of inclusions is considered to be a large parameter.   
%No assumptions of periodicity  have been made, and the asymptotic approximations presented here are uniform with respect to the independent variables. 
The general idea of mesoscale approximations originated a couple of years ago in \cite{MMMeso}, where the Dirichlet 
problem was considered for a domain with multiple inclusions. 


The asymptotic methods, presented here and in  \cite{MMMeso},  can be applied to modelling of dilute composites in problems of mechanics, electromagnetism, heat conduction and phase transition.  %it is 
%They are efficient, in particular, for the situations when %within a perforated solid 
%the boundary conditions have to be satisfied to the required accuracy across a large array of small voids, and when  the approximations commonly used for a finite number of well-separated small voids are not applicable. Our method  will be referred to as the method of 
%{\em mesoscale asymptotic approximations},
%
%We deal with the case of mesoscale approximations for dilute composites, when on one hand the boundary conditions on the boundaries of perforations are satisfied with the required accuracy across a large array of small voids,  and on the other hand the approximations commonly used for a finite number of well-separated small voids are not applicable for the present configuration.  
 %
%As a motivation for the present study, it
% is appropriate to refer
%and for some simple geometries it can be  linked  to physical models of many point interactions.
% which have a wide range of physical applications. %in problems of mechanics, electrostatics, heat conduction and phase transition. 
In such models, the boundary conditions have to be satisfied across a large array of small voids, which is the situation fully served by our approach. Being %applied to 
used in the case of a dilute array of small spherical particles, the method also includes the physical models of many point interactions treated previously in \cite{Figari, FigPapRub, Honig} and elsewhere.
%
%Needless to say, for dilute configurations the point interactions are readily extendable to interactions between small spherical particles, including those cases 
%In particular, a special attention was given in the physics literature to configurations 
%where the number of particles is large and the dilute material  approximations developed for several well-separated small inclusions become inapplicable. Such type of 
Asymptotic approximations applied to solutions of boundary value problems of mixed type in domains containing many small spherical inclusions were considered in \cite{Figari}. The point interaction approximations to solutions of diffusion problems in domains with many small spherical holes were analysed in \cite{FigPapRub}.   Modelling of multi-particle interaction  in problems of phase transition was considered in \cite{Honig} where the evolution of a large number of small 
spherical particles embedded into an ambient medium takes place during the last stage of phase transformation; such a phenomenon where particles in a melt are subjected to growth is referred to as Ostwald ripening. For the numerical treatment of models involving large number $N$ of spherical particles, the fast multipole method, of order $O(N)$,  was proposed    in \cite{Greengard_Rokhlin}, and it appears to be efficient 
 for the rapid evaluation of potential and force fields for systems of a large number of particles  interacting with each other via the Coulomb law.  
 
% We step away from the assumption involving spherical shapes of inclusions, and allow for a wide range of mesoscale geometries: the asymptotic formulae presented here remain efficient even when the typical distance between %the non-spherical 
% perforations of general shape is comparable  to their size.  To take into account the contribution from every perforation, the asymptotic approximation involves a linear combination of dipole fields constructed for individual voids, with the coefficients
 %, which are 
% determined %by solving 
 %from a model linear algebraic system.
 %The formal asymptotic approximations are supplied with the energy estimates for the remainder term.


%In our earlier work  \cite{MMMeso}, we presented asymptotic approximations to solutions of Dirichlet boundary value problems in domains containing a large number of 
%small inclusions. The paper %method of      %mesoscale asymptotic approximations was introduced in 
%\cite{MMMeso}   %, and it 
%%was further applied to 
%also includes the construction and justification of a uniform
%asymptotic approximation of Green's function in a three-dimensional domain with many small inclusions.  
%Similar to the current paper, two geometrical parameters, $\varepsilon$ and $d$, were 
%used to characterize the maximum diameter of inclusions within the array and the minimum %distance 
%separation between the inclusions, respectively.
% The asymptotic approximations
%constructed in \cite{MMMeso}, are efficient for mesoscale geometries, which are intermediate between the case of a finite number of inclusions whose size  is comparable with the distance between the nearest neighbours and the configuration, which gives $\varepsilon \sim \mbox{const}~ d^3$, as appears in the classical homogenization approximations for Dirichlet
%boundary value problems (see, for example,  \cite{CM}, \cite{MKh}).

%Here, we consider an array of small voids, where the geometry is similar to \cite{MMMeso} but the Dirichlet boundary conditions on the surfaces of small impurities have been replaced by the Neumann boundary conditions. The exterior boundary is subjected to the Dirichlet boundary condition. 
%It is shown here that 
%Subject to a weak 
%constraint, $\varepsilon < \mbox{const} ~d$, the mesoscale asymptotic approximation to the solution of the mixed boundary value problem is constructed and rigorously justified. 
%The formal asymptotic approximation is accompanied by the energy estimate of the remainder term.
 
 

 We give an outline of the paper. %main result. 
 The notation $\Omega_N$ will be used for a %bounded 
 domain containing %many 
 small voids $F^{(j)}$, $j=1, \dots, N$, while the %limit
 unperturbed   
 domain, without any holes, is denoted by $\GO$.  The number $N$ is assumed to be large.
 % where $\varepsilon$ is a small positive parameter characterising the normalized diameter of the void. 
 
 If $\GO$ is a bounded domain in ${\Bbb R}^3$, we introduce $L^{1,2}(\GO)$ as the space of functions on $\GO$ with
 distributional first derivatives in $L^2(\GO)$ provided with the norm
 \beq
 \|u\|_{L^{1,2}(\GO)} = \Big(   \|\Grad u \|^2_{L^2(\GO)}  + \| u \|^2_{L^2(\GO)}   \Big)^{1/2}.
 \eequ{norm}
 Here $B$ is a ball at a positive distance from $\prt \GO.$ If $\GO$ is unbounded, by $L^{1,2}(\GO)$ we mean the completion of the space of functions with $\| \Grad u \|_{L^2(\GO)} < \infty,$ which have bounded supports, in the norm \eq{norm}. The space of traces of functions in $L^{1,2}(\GO)$ on $\prt \GO$ will be denoted by $L^{{\tiny 1/2},2}(\prt \GO).$
 
 The maximum of diameters of $F^{(j)}, ~ j=1,\ldots, N$ is denoted by $\Gve$. 
 An array of points $\BO^{(j)}, ~j = 1, \ldots, N, $ is chosen in such a way that
 $\BO^{(j)}$ is an interior point of $F^{(j)}$ for every $j=1,\ldots, N$.
 By $2d$ we denote  the smallest distance between  the points within the array $\{\Oj^{(j)}\}_{j=1}^N$. It is assumed that there exists an open set $\Go \subset \GO$ situated at a positive distance from $\prt \GO$ and such that
 \beq
 \cup_{j=1}^N F^{(j)} \subset \Go, % ~ \mbox{dist} (\prt \Go, \prt \GO) \geq 2h, 
~ \mbox{dist} \big(   \cup_{j=1}^N F^{(j)}, \prt \Go \big) \geq 2d,   ~\mbox{and} ~ \mbox{diam  } \Go = 1,
 \eequ{intro_1}
% where $h>0$ is a constant independent of $\Gve$ and $d$.
%With such a 
With the last normalization of the size of $\Go$, the parameters $\Gve$ and $d$ 
%are 
can be considered as %small
 non-dimensional.
%parameters.  
The scaled %voids 
open sets $\Gve^{-1} F^{(j)}$ are assumed to have %smooth 
%uniformly 
Lipschitz boundaries, with Lipschitz characters independent of $N$. 

Our goal is to obtain an asymptotic approximation to %the 
a unique solution $u_N \in L^{1,2}(\GO_N)$ of the problem
\begin{eqnarray}
-\Delta u_N(\X)=f(\X)\;, \quad \X \in \Omega_N\;,\l{intro_2} \\
u_N(\X)= %0
\phi(\Bx)\;, \quad \X \in \partial \Omega\;,\l{intro_3} \\
 \Dn{u_N}{}(\X)=0\;, \quad \X \in \partial F^{(j)} \;, j=1, \dots, N\;,\l{intro_4}
\end{eqnarray}
where $\phi \in L^{1/2, 2}(\prt \GO)$ and $f (\Bx)$ is a %bounded 
function in $L^\infty(\GO)$ with %a 
compact support %outside 
at a positive distance from the cloud 
$\omega$ of small perforations. %\in C^{0,1}(\ov{\GO}).$

We need solutions to certain model problems in order to construct  the approximation to $u_N$; these include  
\begin{enumerate}
\item $v$ %_f$ 
as the solution of the unperturbed problem in $\Omega$ (without voids),

\item $\BCD^{(k)}$ as the vector function whose components are the dipole fields for the void $F^{(k)}$,

\item $H$ as the regular part of Green's function $G$ in $\Omega$.
\end{enumerate}

%As in \cite{MMMeso}, this 
The approximation relies upon a certain algebraic system, incorporating the field $v_f$ and  integral characteristics associated with the small voids. We define
\[\BGT=\left(\Dxi{v}{1}           %_f}
(\Oj^{(1)}), \Dxi{v}{2}  %_f}
(\Oj^{(1)}),\Dxi{v}{3}  %_f}
(\Oj^{(1)}), \dots,\Dxi{v}{1}  %_f}
(\Oj^{(N)}), \Dxi{v}{2}  %_f}
(\Oj^{(N)}),\Dxi{v}{3}%_f}
(\Oj^{(N)})\right)^T\;,\]
and $%\mathbf{S}
{\frak S}=[\mathfrak{S}_{ij}]_{i, j=1}^N$ %and $\mathbf{P}=[\mathfrak{P}_{ij}]_{i, j=1}^N$, which are 
which is a $3N \times 3N$ matrix  with $3\times 3$ block entries %$\mathfrak{S}_{ij}$ and $\mathfrak{P}_{ij}$:
\[\mathfrak{S}_{ij}=\left\{\begin{array}{ll}\displaystyle{(\nabla_{\bZ} \otimes \nabla_{\bW})\left(G(\Bz, \Bw) %\frac{1}{4\pi|\bZ-\bW|}
\right)\Big|_{\substack{\bZ=\Oj^{(i)}\\ \bW=\Oj^{(j)}}}} & \quad \text{ if } i \ne j\\
0I_3&\quad \text{otherwise}\end{array}  \right., \]
%\[ \mathbf{P}=\diag\{\cP^{(1)}, \dots, \cP^{(N)}\} \]
where $G$ is Green's function in $\GO$, and $I_3$ is the $3 \times 3$ identity matrix.
We also use the block-diagonal matrix
 \beq \mathbf{Q}=\diag\{\BCQ^{(1)}, \dots, \BCQ^{(N)}\}, \eequ{matrix_Q}
where $\BCQ^{(k)}$ is the so-called  $3\times 3$ polarization matrix for the small void $F^{(k)}$ (see 
\cite{MM_Sob} and Appendix G of \cite{MMP}). 
The shapes of the voids $F^{(j)}, j = 1,\ldots, N,$ are constrained in such a way that the maximal and minimal eigenvalues $\Gl_{max}^{(j)}, ~\Gl_{min}^{(j)}$ of the matrices $-\BCQ^{(j)}$ satisfy the inequalities
\beq
A_1 \Gve^3 > \max_{1 \leq j \leq N} \Gl_{max}^{(j)}, ~~ % \geq 
\min_{1 \leq j \leq N} \Gl_{min}^{(j)} > A_2 \Gve^3, % > 0,
\eequ{Gl_min} 
where %the constants 
$A_1$ and  $A_2$ are positive and independent of $\Gve$.

%As the main result of the paper, we prove
One of the results, for the case when $\GO={\Bbb R}^3$, $H\equiv 0$, and when \eq{intro_3} is replaced by the condition of  decay 
of $u_N$ at infinity, 
can be formulated as follows

\vspace{0.1in}
%\begin{thrm}
\begin{thm}
 \label{thm1_alg_f_inf} 
Let  %the parameters $\varepsilon$ and $d$ satisfy the inequality
\[\varepsilon < c\, d\;,\]
where $c$ is a sufficiently small absolute constant. Then the solution $u_N(\X)$ 
admits the asymptotic representation
%is defined by the asymptotic formula
\begin{equation}\label{introeq1}
u_N(\X)=v%_f
(\X)+%\varepsilon 
\sum^N_{k=1} \boldsymbol{C}^{(k)} \cdot %\left\{ 
\BCD^{(k)}(\Bx) %(\varepsilon^{-1}(\X-\Oj^{(k)}))+\varepsilon^2 \cP
%-%+
%\BCQ^{(k)} \nabla_\Y H(\X, \Oj^{(k)})  \right\}
+\CR_N(\X)\;,
\end{equation}
where $\boldsymbol{C}^{(k)}=(C^{(k)}_1, C^{(k)}_2, C^{(k)}_3)^T$ and  the column vector $\mathbf{C}=(C^{(1)}_1, C^{(1)}_2, C^{(1)}_3, \dots, C^{(N)}_1, C^{(N)}_2, C^{(N)}_3)^T$ %solves 
satisfies the invertible linear
algebraic system 
\beq
(\mathbf{I}+ %\varepsilon^3 
%\mathbf{S}
{\frak S} \mathbf{Q})\mathbf{C}  = -\BGT\;.
\eequ{alg_s_intro}
The 
%matrix $(\mathbf{I}-%\varepsilon^3 
%%\mathbf{S}
%{\frak S} \mathbf{Q})$ is invertible and the 
remainder $\CR_N$ satisfies the energy
estimate
\begin{equation}\label{introeq2}
 \| \nabla \CR_N\|^2_{L_2(\Omega_N)} \le \text{\emph{const} } \Big\{ \varepsilon^{11%8
 }d^{-11%8
 } + \varepsilon^{5}d^{-3} \Big\} \| \nabla v%_f
 \|^2_{L^2( \GO % {\Bbb R}^3  %\omega
 )}  %+ d^2  \|  v_f\|^2_{L_2(\omega_h)}  
 %\Big\}
  .%+   %\varepsilon
 %\,d^{2}\max_{1 \le i, j \le 3}\Big\| \frac{\partial^2 v_f}{\partial x_i \partial x_j} \Big\|^2_{L_\infty(\omega)}\Big\}\;.
 \end{equation}
 %where $\Go_h$ stands for the extended cloud region occupied by small voids.
%\end{thrm}
\end{thm}
We remark that since $\Gve$ and $d$ are non-dimensional parameters,  there is no dimensional mismatch in the right-hand side of \eq{introeq2}.

We now describe the plan of the article. In Section \ref{MainNotmeso}, we introduce the multiply-perforated geometry and
% the corresponding notations.
% whose solution we will derive the asymptotic approximation. 
%The 
consider the above model problems.
%, whose solutions are used in the asymptotic approximation. %, are defined in Section  \ref{Modelproblems}.
%After specifying model solutions used in the construction of this approximation in Section \ref{Modelproblems}, our objective is formally carried out initially for the simpler case of an unbounded domain with many small voids in Section \ref{R3alg}.
% with the aim of illustrating features of 
The formal asymptotic algorithm for a cloud of small perforations in the infinite space and the analysis of the algebraic system
\eq{alg_s_intro} are given in Sections \ref{R3alg} and \ref{alg_syst}. Section \ref{R3energyesy} presents the 
proof of Theorem \ref{thm1_alg_f_inf}. %  remainder estimate.
The problem for a cloud of small perforations in a general 
% bounded 
domain is considered in Section \ref{boundformalg}. 
%The asymptotic approximation presented there remains valid for an arbitrary three-dimensional perforated domain.  
 Finally, in Section \ref{example} we give an illustrative example accompanied by the numerical simulation.

 %This asymptotic algorithm 
% will be extended in subsequent sections for situation of the bounded domain. Justification of the asymptotics presented in Section \ref{R3alg} is then given in Section \ref{R3energyesy}. We consider the formal asymptotic approximation of a solution to the mixed problem in a bounded domain with many voids in Section \ref{boundformalg}, and using the techniques implemented in Section \ref{R3energyesy}, we provide the energy estimate for the remainder produced in this approximation.
 % in Section \ref{boundenergyestRN}.




==> Mesoscale pdf/Mainnot_meso.tex <==
\section{Main notations and model boundary value problems}\label{MainNotmeso}
%Here 
Let  $\Omega$ be a  bounded 
domain in $\mathbb{R}^3$ with a smooth boundary $\prt \GO$. We shall also consider the case when $\GO = {\Bbb R}^3 .$  

%If it is bounded, we assume that  the boundary $\partial \Omega$ is smooth.  %and compact closure $\bar{\Omega}$. We denote by $\omega^{(j)}$ a subset of $\mathbb{R}^3$, with smooth boundary $\partial \omega^{(j)}$ and compact closure $\overline{\omega^{(j)}}$, whose complement in the infinite space is $C\omega^{(j)}=\mathbb{R}^3\backslash \overline{\omega^{(j)}}$, $j=1, \dots, N$. The sets $\omega^{(j)}$, $j=1, \dots, N$, are assumed to contain the origin $\Oj$, and the diameter of each of these sets is 1.
%Let $\omega_\varepsilon^{(j)}$ be a subset of $\Omega$ with centre $\Oj^{(j)}$, $1 \le j \le N$. We relate the domain $\omega^{(j)}_\varepsilon$ to  $\omega^{(j)}$ via $\omega_\varepsilon^{(j)}=\{\X:\varepsilon^{-1} (\X-\Oj^{(j)}) \in \omega^{(j)}\}$, $j=1, \dots, N$. Here, $\varepsilon$ is one of the small positive parameters used in the present article and this characterizes the normalized diameter of the void $\omega_\varepsilon^{(j)}$, $j=1, \dots, N$, the other parameter being 
%\[ d=2^{-1} \min_{i \ne j, 1 \le i, j\le N}|\Oj^{(j)}-\Oj^{(i)}|\;,\]
% and we assume  that $\varepsilon < c\, d$, with $c$ being a sufficiently small constant. The number $N$ of voids is assumed to be large.
%
% We introduce the domain $\omega\subset \Omega$, whose diameter is equal to 1, and such that 
 %\[ \bigcup_{j=1}^N \omega_\varepsilon^{(j)} \subset \omega\;.\] 
% Additional assumptions also made on $\omega$ are 
 %\[ \text{dist}(\partial \omega, \partial \Omega) \ge 2 d\;, \quad \text{ and }\quad \text{dist} \big\{ \bigcup_{j=1}^N \omega_\varepsilon^{(j)}, \partial \omega\big\}\ge 2d\;.\]
 The perforated domain $\Omega_N$, % in which we aim to give an asymptotic approximation of $u_N$ 
 is given by
 \[\Omega_N=\Omega \backslash \overline{\cup_{j=1}^N F^{(j)}}\;,\]
 where  $F^{(j)}$ are small voids introduced in the previous section. Also in the previous section we introduced the notations $\Gve$ and $d$ for two small parameters, characterizing the maximum of the diameters of
 $F^{(j)}, j=1,\ldots,N,$ and the minimal distance between the small voids, respectively.  
% In subsequent sections, along with $\X$ we associate the scaled variable $\XI_j=\varepsilon^{-1}(\X-\Oj^{(j)})$. 
%The notation $g=O(f)$ represents the inequality $g\le \text{const }|f|$. 
 
 In sections where we are concerned with the energy estimates of the remainders produced by asymptotic approximations we %will 
 frequently use the obvious estimate
 \begin{equation}\label{sumestvd}
 N \le \text{const }d^{-3}\;.
 %\sum_{k=1}^N 1 \le \text{const }d^{-3} \text{meas}_3(\omega) \le \text{const }d^{-3}\;,  
 \end{equation}
% where $\text{meas}_3(\omega)$ is the three-dimensional measure of $\omega$ and this estimate is deduced by considering the sum on the left hand side as a Riemann integral over the cloud of inclusions $\omega$. 
 
 We %dedicate our attention
 % in the first part of this article,
  %to 
  consider the approximation of  the function 
  $u_N$ which is a variational solution of the mixed problem \eq{intro_2}-\eq{intro_4}.
 %\begin{equation}\label{Mainnot1}
 %-\Delta u_N(\X)=f(\X)\;, \quad \X \in \Omega_N\;,
 %\end{equation}
 %\begin{equation}\label{Mainnot2}
 % u_N(\X)=0\;, \quad \X \in \partial \Omega\;,
  %\end{equation}
  %\begin{equation}\label{Mainnot3}
   %\Dn{u_N}{}(\X)=0\;, \quad \X \in \partial \omega^{(j)}_\varepsilon\;, j=1, \dots, N\;.
   %\end{equation}
  % where $f$ is assumed to be a %smooth 
  % bounded 
   %function with a compact support in $\Omega \setminus \ov{\Go}$.
   %, such that $\text{diam }(\text{supp }f) \le C$, with $C$ being an absolute constant and $\text{supp }f \cap \omega=\varnothing$. 
   %It is also assumed that $\mbox{dist } (\Go, \mbox{supp } f) > h > 0,$ where the constant $h$ is independent of $\Gve$ and $d$.  
%   The notation $\Go_h$ will be used for a bounded domain, which includes $\Go$, and such that
 %  %Here $\partial /\partial n=\N^{(j)} \cdot \nabla $ is the normal derivative, with $\N^{(j)}$ being the unit outward normal to %%$\omega_\varepsilon^{(j)}$, $j=1, \dots, N$.
 %  \beq
 %  \Go_h = \{ \Bx: \mbox{dist }(\omega, \Bx) < h \}.
  % \eequ{om_h}
   
     
 

==> Mesoscale pdf/Meso_bibliography_1.tex <==
\begin{thebibliography}{8}
%\bibitem{CM} Cioranescu, D., Murat, F., \emph{A strange term brought from somewhere else}, Nonlinear Partial Differential Equations and their Applications, Coll\`ege de France Seminar, Vol. II and III. Research Notes in Mathematics, 60 and 70, 98--138 and 154--178 (1982).
\bibitem{Figari} Figari, R., Theta, A. \emph{A boundary  value problem of mixed type on perforated domains.} Asymptotic Anal., 6, 271-284 (1993). 
\bibitem{FigPapRub} Figari, R., Papanicolaou, G., Rubinstein, J., \emph{The point interaction approximation for diffusion in regions
with many small holes. } Stochastic Methods in Biology. Lecture Notes in Biomaterials, Vol. 70, 75-86 (1987).
\bibitem{Greengard_Rokhlin}  Greengard, L.,  Rokhlin,  V., {\it A fast algorithm for particle simulations.}   Journal of Computational Physics, { 73}, 325--348  (1987).
\bibitem{Honig} H\"{o}nig, A., Niethammer, B., Otto, F., \emph{On first-order corrections to the LSW theory I: Infinite systems.}
Journal of Statistical Physics, 119, 61-122 (2005).
\bibitem{MKh} Marchenko, V. A., Khruslov, E. Ya., \emph{Homogenization of Partial Differential Equations}, Birkh\"auser (2006).
\bibitem{MMMeso} Maz'ya, V., Movchan, A. \emph{Asymptotic treatment of perforated domains without homogenization}, Mathematische Nachrichten (to appear).
\bibitem{MM_Sob} Maz'ya, V., Movchan, A. \emph{Uniform asymptotics of Green's kernels for mixed and Neumann problems in domains with small holes and inclusions}, In: Sobolev Spaces in Mathematics III. Applications in Mathematical Physics. pp. 277-316, Springer, 2009.
%\bibitem{Mikhlin} Mikhlin, S.G., \emph{The course of mathematical physics}, Nauka, Moscow (1968).
\bibitem{MMP} Polya, G.,  Szeg\"o G., \emph{Isoperimetric inequalities in mathematical physics}, Princeton University Press, Princeton (1951).
%Movchan, A. B., Movchan, N. V., Poulton, C. G.: \emph{Asymptotic Models of Fields in Dilute and Densely packed composites}, Imperial College Press, (2002).
\bibitem{SP} Sanchez-Palencia, E., \emph{Non-homogeneous media and vibration theory}, Springer-Verlag, New York (1980).
\bibitem{stein} Stein, E.M., \emph{ Singular integrals and differentiability properties of functions}, Princeton University Press, Princeton (1970).
\end{thebibliography}

==> Mesoscale pdf/Model_problems.tex <==
%\section{Model boundary value problems}
\label{Modelproblems}
Before constructing the approximation to $u_N$, we introduce model auxiliary functions which the asymptotic scheme relies upon.

\begin{enumerate}
\item \emph{%The s
Solution $v$ %_f$ 
in the unperturbed domain $\Omega$.} Let $v%_f
\in L^{1,2}(\GO)$ denote a %the 
unique variational solution of the problem
\begin{eqnarray}
-\Delta v%_f
(\X)&&=f(\X)\;, \quad \X \in \Omega\;,\l{vfom_1} \\
 v%_f
 (\X)&&= \phi(\Bx)
 %0
 \;, \quad \X \in \prt \Omega\;.  \l{vfom_2}   \end{eqnarray}

\item \emph{%The r
Regular part of Green's function in $\Omega$.} By $H$ we mean the regular part of Green's function $G$ in $\Omega$ defined by the formula
\beq H(\X, \Y)=(4\pi|\X-\Y|)^{-1}-G(\X, \Y)\;.\eequ{H_def}
Then $H$ is a variational solution of 
\[ \Delta_\X H(\X, \Y)=0\;, \quad \X, \Y \in \Omega\;,\]
\[ H(\X, \Y)=(4\pi|\X-\Y|)^{-1}\;, \quad\X \in \partial \Omega, \Y \in \Omega\;.\]

\item \emph{The dipole fields $\cD^{(j)}_i, ~ i=1, 2, 3,$ associated with the  void $F^{(j)}$.} The vector functions $\BCD^{(j)}=\{ \cD^{(j)}_i\}^3_{i=1}$, %whose components are 
which are called the dipole fields,  %solve the problems
are variational solutions of the exterior Neumann problems
%is responsible for solving 
\begin{equation}\label{modfieldeq1}
\left. \begin{array}{c}
\displaystyle{\Delta \BCD^{(j)}(\Bx)=\Oj\;, \quad \Bx \in %C
{\Bbb R}^3 \setminus \bar{F}^{(j)}\;,}\\
\displaystyle{ \Dn{\BCD^{(j)}}{}(\Bx)=\N^{(j)}\;,\quad \Bx \in \partial F^{(j)}\;,}\\
\displaystyle{ \BCD^{(j)}(\Bx)=O(\varepsilon^3 |\Bx-\BO^{(j)}|^{-2}) \quad \text{ as }\quad | \Bx | \to \infty \;,}
\end{array}\right\}
 \end{equation}
where $\N^{(j)}$ is the unit outward normal with respect to $F^{(j)}$.
In the text below we also use %the notion of 
the %dipole 
negative definite polarization matrix $\BCQ^{(j)}=\{\CQ^{(j)}_{ik}\}_{i, k=1}^3$,
as well as the following asymptotic result (see \cite{MM_Sob} and Appendix G in \cite{MMP}), for every  void $F^{(j)}$:

\begin{lem}\label{Djasymp}
For $|\Bx - \BO^{(j)}|>2 \Gve$, the dipole fields admit the asymptotic representation
\begin{equation}\label{modfieldeq2}
\cD^{(j)}_i(\Bx)=\frac{1}{4\pi} \sum^3_{m=1} \CQ^{(j)}_{im} \frac{x_m- O^{(j)}_m}{|\Bx - \BO^{(j)}|^3}+O\left(\Gve^{4} {|\Bx-\BO^{(j)}|^{-3}}\right)\;, \quad i=1,2,3\;.
\end{equation}
%where $\max_{i,j} |\CQ^{(j)}_{im}| \leq \mbox{\rm const}~ \Gve^3.$
\end{lem}

The shapes of the voids $F^{(j)}, j = 1,\ldots, N,$ are constrained in such a way that the maximal and minimal eigenvalues $\Gl_{max}^{(j)}, ~\Gl_{min}^{(j)}$ of the matrices $-\BCQ^{(j)}$ satisfy the inequalities \eq{Gl_min}.
%\beq
%A_1 \Gve^3 > \max_{1 \leq j \leq N} \Gl_{max}^{(j)} \geq \min_{1 \leq j \leq N} \Gl_{min}^{(j)} > A_2 \Gve^3 > 0,
%\eequ{Gl_min} 
%where the constants $A_1, A_2$ are independent of $\Gve$.

%We shall also use the notation \beq \BCP_\Gve^{(j)} = \Gve^3 \BCP^{(j)} \eequ{P_eps} for the polarization matrix of the small (unscaled) inclusion $\Go_\Gve^{(j)}$.
\end{enumerate}



==> Mesoscale pdf/Numerical_scheme.tex <==
\subsection{Non-uniform cloud containing a large number of spherical voids}

Here we consider the same mixed boundary value problem as in Section \ref{cloud_example}, but the cloud of voids is chosen in such a way that the number $N$ may be large and voids of different radii are distributed in a non-uniform arrangement.
For different values of $N$, the overall volume of voids is preserved - examples of the clouds used here are shown in Fig.
\ref{diagramcloud}.

The results  are based on the numerical implementation of formula (\ref{introeq1a}) in MATLAB.

%Here we will implement (\ref{introeq1a}) in a numerical scheme developed in MATLAB. We consider a different geometry for $\Omega_N$ used in the first example, which we now describe.
%
%\subsubsection*{The cloud $\omega$} Let the set 
The cloud $\omega$ %be 
is assumed to be the cube with side length $\frac{1}{\sqrt{3}}$ and the centre at $(3, 0, 0)$. 
Positioning of voids is described as follows. Assume we have $N=m^3$ voids, where $m=2,3, \dots$.
 % we divide 
 Then $\omega$ is divided into   %$N=m^3$, $m=1,2, \dots$, 
 $N$ smaller cubes of side length $h=\frac{1}{\sqrt{3}m}$, and the centres of voids are placed at% Next, we position voids with centres 
\[\BO^{(p,{q,r})}=\Big(3-\frac{1}{2\sqrt{3}}+\frac{2p-1}{2}h,-\frac{1}{2\sqrt{3}}+\frac{2q-1}{2}h, -\frac{1}{2\sqrt{3}}+\frac{2r-1}{2}h\Big) \]
for $p, q, r=1, \dots, m$, and we assign their radii $\rho_{p,{q,r}}$ by
\[\rho_{p,{q,r}}=\left\{\begin{array}{ll}
\displaystyle{\frac{h}{5}} &\quad \text{if }{p>q}\;,\\
\displaystyle{\frac{\alpha h}{2}}& \quad \text{if } p<q\;,\\
\displaystyle{\frac{h}{4} }& \quad \text{if } p=q\;,
\end{array}\right.\]
where $\alpha <1$, % is prescribed to be less than $1$, and is discussed in detail below.
and it is chosen in such a way that the overall volume of all voids within the cloud remains constant for different $N$.
An elementary calculation suggests that there will be $m^2$ voids with radius $\frac{h}{4}$ and equal number $\frac{m^2(m-1)}{2}$ of voids with radius $\frac{h}{5}$ or $\frac{\Ga h}{2}$.

%In our experiment, we will aim to increase the number of voids $N$ without changing the volume of which the total number of small spherical voids occupy in the cube $\omega$. Suppose the fraction of the volume occupied by the voids in $\omega$ is $\beta$. Then, 
Assuming that the volume fraction of all voids within the cube is equal to $\beta$, we have
%we have the total volume the voids occupy is given by the formula
\[\frac{4\pi h^3}{3} \Big(\frac{m^2(m-1)(8+125 \alpha^3)}{2000}+\frac{m^2}{64}\Big)=\beta \frac{1}{3\sqrt{3}}\;,\]
%Recalling that $h=\frac{1}{\sqrt{3}m}$, after rearrangement we obtain 
and hence
\begin{equation}\label{alphaeq}
\alpha^3=\frac{16m}{m-1}\Big\{\frac{3}{4\pi}\beta -\frac{125+32(m-1)}{8000 m}\Big\}\;.
\end{equation}
%Allowing $m$ to tend to infinity, one obtains 
%that $\beta$ should satisfy 
In particular, if $N \to \infty$, the limit value $\Ga_\infty$ becomes
\begin{equation}\label{alphainf}
\alpha_\infty=\Big\{\frac{12}{\pi}\beta -\frac{8}{125}\Big\}^{1/3}\;.
\end{equation}
%Thus,  in order that $ \alpha <1$, we should choose $\beta$ so that
%\[\beta< \left\{\frac{133\pi}{1500}\right\}^{1/3}\;.\]
In the numerical computation of this section, $\beta = \pi/25.$
%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.495\textwidth]{Nvalpha.eps}
%\caption{The graph of $\alpha$ versus $N$ given by formula when $\beta= \pi/25$, for large $N$ we see that $\alpha$ tends to 0.7465 which is predicted value present in (\ref{alphainf}). }
%\label{fig3}
%\end{figure}

%\subsubsection*{Numerical scheme} We choose $\beta=4\pi/100$ , 
Taking $R=7$ and $\rho=2$, we %and consider plotting 
compute the leading order approximation of $u_N-v$, as defined  in the  asymptotic formula (\ref{introeq1a}), along the line $\gamma$ at the intersection of the planes $x_2=-1/(2\sqrt{3})$ and $x_3=-1/(2\sqrt{3})$, for $N=8, 125, 1000$. Fig. \ref{fig4} below shows the configuration of the cloud of voids for a) $N=8$ and b) $N=125$. For a large number of voids $(N=1000)$,  Fig. \ref{fig4a}a) shows the cloud and Fig \ref{fig4a}b) includes the graph of $\alpha$ versus $N$. The plot of $u_N-v$ given by (\ref{introeq1a}) for $2\le x_1\le 4$ is shown in Fig. \ref{fig5}. The asymptotic correction has been computed along the straight line $\gamma=\{ x_1 \in \mathbb{R}, x_2=-1/(2\sqrt{3}),  x_3=-1/(2\sqrt{3})\}$. Dipole type fluctuations are clearly visible on the diagram. Beyond $N=1000$ the graphs are visually indistinguishable and hence the values $N=8, 125, 1000$, as in Figures \ref{fig4} and \ref{fig4a} have been chosen in the computations. The algorithm is fast and does not impose periodicity constraints on the array of small voids.
   \begin{figure}[htbp]
\begin{minipage}[b]{0.495\linewidth}
\centering
\includegraphics[width=\textwidth]{cloud8pdf.pdf}

a)
\end{minipage}
\begin{minipage}[b]{0.495\linewidth}
\centering
\includegraphics[width=\textwidth]{Cloud125pdf.pdf}


b)
\end{minipage}
\caption{The cloud of voids for the cases when a) $N=8$ and b) $N=125$.}
\label{fig4}
\end{figure}


 \begin{figure}[htbp]
\begin{minipage}[b]{0.495\linewidth}
\centering
\includegraphics[width=\textwidth]{Cloud1000pdf.pdf}

a)
\end{minipage}
\begin{minipage}[b]{0.495\linewidth}
\centering
\includegraphics[width=\textwidth]{Nvalphapdf.pdf}


b)
\end{minipage}
\caption{a) The cloud of voids for the cases when $N=1000$, b) The graph of $\alpha$ versus $N$ given by formula (\ref{alphaeq}) when $\beta= \pi/25$, for large $N$ we see that $\alpha$ tends to 0.7465 which is predicted value present in (\ref{alphainf}).}
\label{fig4a}
\end{figure}

 \begin{figure}[htbp]
\centering
\includegraphics[width=0.7\textwidth]{uNminusVpdf.pdf}
\caption{The graph of $u_N-v$ given by (\ref{introeq1a}), for $2 \le x_1\le 4$ plotted along the straight line $\gamma$ adjacent to the cloud of small voids.}
\label{fig5}
\end{figure}

\vspace{0.1in}\emph{Acknowledgments. }We would like to acknowledge the financial support of the U.K. Engineering and Physical Sciences Research Council through the research grant EP/F005563/1.

==> Mesoscale pdf/R3alg_m.tex <==
\section{The formal approximation of $u_N$ for the infinite space containing many voids}\label{R3alg}
%Before proving Theorem stated in the Introduction for a bounded domain, we consider a simpler 
%Here, we consider the situation when $\Omega=\mathbb{R}^3$.
%, for simplicity, we first consider the situation when $\Omega=\mathbb{R}^3$, where the results obtained here will be used in the case when $\Omega_N$ is bounded.

In this section we deduce formally the uniform asymptotic approximation of $u_N$: 
\[ u_N(\X)\sim v%_f
(\X)+ %\varepsilon 
\sum^N_{k=1} \boldsymbol{C}^{(k)} \cdot \BCD^{(k)}(\Bx %\XI_k
)\;,\] 
for the case $\Omega=\mathbb{R}^3$ and derive an algebraic system for %that is satisfied by 
the coefficients $\boldsymbol{C}^{(k)}=\{C^{(k)}_i\}^3_{i=1}$, $k=1, \dots, N$.

%Then, in this case, 
The function $u_N$ satisfies
\begin{equation}\label{R3formalgeq1}
-\Delta u_N(\X)=f(\X)\;, \quad \X \in \Omega_N\;,
\end{equation}
\begin{equation}\label{R3formalgeq2}
\Dn{u_N}{}(\X)=0\;,\quad \X \in  \partial F%\omega_\varepsilon
^{(j)}, j=1, \dots, N\;,
\end{equation}
\begin{equation}\label{R3formalgeq3}
u_N(\X)\to 0\;, \quad \text{ as }|\X| \to \infty\;.
\end{equation}
%Since $\text{supp }f \cap \omega=\varnothing$, 
%The right-hand side (\ref{R3formalgeq1}) is subject to the condition
%\begin{equation}\label{R3formalgeq4}
%\int_{\mathbb{R}^3} f(\X)\, d\X=0\;.
%\end{equation}
We begin by constructing the %first order approximation 
asymptotic representation for $u_N$ in this way
\begin{equation}\label{R3formalgeq5}
u_N(\X)=v%_f
(\X)+     %\mathcal{R}^{(1)}_N(\X)\;,
\sum^N_{k=1} \boldsymbol{C}^{(k)} \cdot \cD^{(k)}(\Bx)+\mathcal{R}_N(\X)\, 
\end{equation}
where $\CR_N$ is the remainder, and $v%_f
(\X)$ satisfies
\[ -\Delta v%_f
(\X)=f(\X)\;, \quad \X \in \mathbb{R}^3\;,\]
\[ v%_f
(\X) \to 0 \quad \text{ as } \quad |\X| \to \infty\;,\]
%\[\int_{\mathbb{R}^3} f(\X)\, d\X=0\;.\]
and $\cD^{(k)}$ are the dipole fields defined as solutions of problems \eq{modfieldeq1}.
%Then $\mathcal{R}^{(1)}_N$, appearing in (\ref{R3formalgeq5}), is a harmonic function in $\Omega_N$ which decays at infinity. Considering the normal derivative on the small void $%\omega_\varepsilon
%F^{(j)}$, $j=1, \dots, N$ we have
%\begin{eqnarray}\nonumber\label{R3formalgeq6}
%\Dn{\mathcal{R}^{(1)}_N}{}(\X)&=&-\N^{(j)}\cdot \nabla v_f(\X)\\
%&=&-\N^{(j)}\cdot \nabla v_f(\Oj^{(j)})+O(\varepsilon)\;, \quad \X \in \partial F%\omega
%^{(j)}%_\varepsilon
%, j=1, \dots, N\;.
%\end{eqnarray}
%A linear combination of the dipole fields introduced in Problem 3 of Section 3 is now used to correct for the discrepancy
%in the preceding boundary conditions and construct $\mathcal{R}^{(1)}_N$:
%\begin{equation}\label{R3formalgeq7}
%\mathcal{R}^{(1)}_N(\X)=%\varepsilon 
%\sum^N_{k=1} \boldsymbol{C}^{(k)} \cdot \cD^{(k)}(\Bx)+\mathcal{R}_N(\X)\;,  
%\end{equation}
%where 
The function $\mathcal{R}_N$ is harmonic in $\Omega_N$ and 
\begin{equation}\label{R3formalgeq8}
\mathcal{R}_N(\X) =O(|\X|^{-1}) \quad \text{ as } |\X| \to \infty\;.
\end{equation}
Placement of (\ref{R3formalgeq5%7
}) into (\ref{R3formalgeq2%6
}) together with (\ref{modfieldeq1}) gives the boundary condition on $\prt F^{(j)}$:
\[\Dn{\mathcal{R}_N}{}(\X)=-\N^{(j)} \cdot \Big\{ \nabla v%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)}+O(\varepsilon)+ %\varepsilon 
\sum_{\substack{k \ne j\\ 1 \le k \le N}} \nabla (\boldsymbol{C}^{(k)} \cdot \cD^{(k)}(\Bx))\Big\} .
% \;, \quad \X \in  \partial %\omega_\varepsilon
%F^{(j)}, j=1, \dots, N\;.
\]
Now we use (\ref{modfieldeq2}), for $\cD^{(k)}$, $k \ne j$, so that this boundary condition becomes
\begin{eqnarray*}
\Dn{\mathcal{R}_N}{}(\X)&\sim&
-\N^{(j)}\cdot\Big\{ \nabla v%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)}%+O(\varepsilon) -\varepsilon^3 
+\sum_{\substack{k \ne j \\ 1 \le k \le N}} T(\X, \Oj^{(k)})\BCQ^{(k)} \boldsymbol{C}^{(k)} \Big\}%\\
%&&+O\Big(\sum_{\substack{k \ne j \\ 1 \le k \le N}} \frac{\varepsilon^4 |\boldsymbol{C}^{(k)}|}{|\X -\Oj^{(k)}|^4}\Big) \Big\}
\;, \quad \X \in \partial F^{(j)}, j=1, \dots, N\;,
\end{eqnarray*}
where
\begin{equation}\label{defT}
T(\X, \Y)=(\nabla_{\bZ} \otimes \nabla_{\bW})\left( \frac{1}{4\pi|\bZ-\bW|}\right)\Big|_{\substack{\bZ=\X\\ \bW=\Y}}\;.
\end{equation}
Finally, Taylor's expansion of $T(\X, \Oj^{(k)})$ about $\X=\Oj^{(j)}, ~ j \neq k, $ leads to 
\begin{eqnarray*}
\Dn{\mathcal{R}_N}{}(\X)&\sim&
-\N^{(j)}\cdot\Big\{ \nabla v%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)}%+O(\varepsilon) -\varepsilon^3 
+\sum_{\substack{k \ne j \\ 1 \le k \le N}} T(\Oj^{(j)}, \Oj^{(k)})\BCQ^{(k)} \boldsymbol{C}^{(k)} %\\
%&&+O\Big(\sum_{\substack{k \ne j \\ 1 \le k \le N}} \frac{\varepsilon^4 |\boldsymbol{C}^{(k)}|}{|\Oj^{(j)} -\Oj^{(k)}|^4}\Big) 
\Big\}\;, \quad \X \in \partial %\omega_\varepsilon
F^{(j)}, j=1, \dots, N\;.
\end{eqnarray*}
%Upon considering removing 
To remove the leading order discrepancy in the above boundary condition, %gives rise to 
we require that the vector coefficients $\BC^{(j)}$ satisfy the algebraic system
\begin{equation}\label{R3formalgeq9}
\nabla v%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)}+%\varepsilon^3 
\sum_{\substack{ k \ne j \\ 1 \le k \le N}} T(\Oj^{(j)}, \Oj^{(k)})\BCQ^{(k)}\boldsymbol{C}^{(k)}=\Oj\;, \quad \text{ for } j=1, \dots, N\;,
\end{equation} 
where the polarization matrices $\BCQ^{(j)}$ %_\Gve$, defined in \eq{P_eps} 
characterize the geometry of %the small voids $%\Go_\Gve
$F^{(j)}, ~ j= 1, \ldots, N.$ 
Upon solving the above algebraic system, the formal asymptotic approximation of $u_N$ is complete. The next section addresses the solvability of the system   \eq{R3formalgeq9}, together with %the 
estimates  for
the vector coefficients $\BC^{(j)}.$ 



==> Mesoscale pdf/R3energyesy.tex <==
\section{
%Approximation of $u_N$ in $\mathbb{R}^3 \backslash \overline{\cup_{j=1}^N F %\omega_\varepsilon
%^{(j)}}$
Energy error estimate in the case $\GO= {\Bbb R}^3$}\label{R3energyesy}
In this section we %give the main 
prove the result concerning the asymptotic approximation of $u_N$ for the 
%unbounded 
perforated domain $\Omega_N=\mathbb{R}^3 \backslash \overline{\cup_{j=1}^N F%\omega_\varepsilon
^{(j)}}$. The changes in the argument, necessary for the treatment of a general domain, will be described in
Section \ref{boundformalg}.  
%\begin{thm}\label{R3thmasy}
%Let the small parameters $\varepsilon$ and $d$ defined in Section $\ref{MainNotmeso}$, satisfy the inequality
%\[\varepsilon< c\, d   , \] % |\log d|^{-1/3}\;,\]
%where $c$ is a sufficiently small absolute constant. Then the matrix $\mathbf{I}- %\varepsilon^3 
%\BCS \mathbf{Q}$ defined in Section $\ref{R3alg}$ is invertible and the solution $u_N(\X)$ to the problem $(\ref{R3formalgeq1})$--$(\ref{R3formalgeq3})$ is defined by the asymptotic formula
%\begin{equation}\label{R3energyest1}
%u_N(\X)=v_f(\X)+%\varepsilon 
%\sum_{k=1}^N \boldsymbol{C}^{(k)}\cdot \BCD^{(k)}(\Bx)+\mathcal{R}_N(\X)\;,
%\end{equation}
%where $\boldsymbol{C}^{(k)}=(C^{(k)}_1, C^{(k)}_2, C^{(k)}_3)^T$ solve the algebraic system {\rm \eq{alg1}}.%and the entries $C^{(k)}_i$ are given by $(\ref{R3formalgeq10})$. 
%The remainder $\mathcal{R}_N$ satisfies the energy estimate
%\begin{equation}\label{R3energyest2}
% \| \nabla \mathcal{R}_N\|^2_{L_2(\Omega_N)} \le \text{\emph{const} } \Big\{ \varepsilon^{11%8
% }d^{-11%8
% } + \varepsilon^{5}d^{-3} \Big\}  \| \nabla v_f\|^2_{L_2(   %\omega
%{\Bbb R}^3 )} %+ d^2  \big\| v_f \big\|^2_{L_2(\Go_h)} \Big\}  ,
% %+d^2 \max_{1 \le i, j \le 3}\Big\| \frac{\partial^2 v_f}{\partial x_i \partial x_j} \Big\|^2_{L_\infty(\omega)}\Big\}
 %\;.
% \end{equation}
%% where $\Go_h$ is the extended cloud occupied by small voids, as defined in {\rm \eq{om_h}}.
%\end{thm}

%\begin{proof}
{\em Proof of Theorem {\rm \ref{thm1_alg_f_inf}}.}
\emph{a) %The problem 
Neumann problem for the remainder.} The remainder term  $\CR_N$ in %\eq{R3energyest1} 
\eq{introeq1} is a harmonic function in $\GO_N$, which vanishes at infinity and satisfies the % following  
boundary conditions % on the surfaces of small voids: 
\beq
\fr{\prt \CR_N}{\prt n}(\Bx) = - \Big(\Grad v(\Bx) + \BC^{(j)} \Big) \cdot \boldsymbol{n}^{(j)}(\Bx) - \sum_{\substack{ k \neq j \\ 1 \leq k \leq N}} \BC^{(k)} \cdot \fr{\prt}{\prt n} \BCD^{(k)}(\Bx), %\BGx_k), 
~~\mbox{when}~~ \Bx \in \prt %\Go_\Gve
F^{(j)}, j = 1, \ldots, N.
\eequ{rem1} 
Since $\mbox{supp } f $ %has an empty intersection with 
is separated from $%\ov{\Go}_\Gve
F^{(j)}, j = 1, \ldots, N,$ and since $\BCD^{(j)}, ~j =1,\ldots,N,$ satisfy  \eq{modfieldeq1} we have 
\beq
\int_{\prt %\Go_\Gve
F^{(j)}}  \fr{\prt \CR_N}{\prt n}(\Bx) dS_\Bx = 0, ~ j=1,\ldots, N.
\eequ{rem2}
\emph{b) Auxiliary functions.} Throughout the proof we use the notation $B^{(k)}_\rho=\{\X:|\X-\Oj^{(k)}|<\rho\}$.
% and $B_R=\{\X:|\X%-\Oj
%|<R\}$,  where $R$ is sufficiently large and  $\text{dist}(\omega, \partial B_R)>2d$. 
We %begin by introducing 
introduce %some 
auxiliary functions which will help us to obtain %(\ref{R3energyest2}). 
\eq{introeq2}. Let 
\begin{eqnarray} \nonumber
\Psi_k(\X)&=&v%_f
(\X)
-v%_f
(\BO^{(k)})-(\X-\Oj^{(k)})\cdot \nabla v(\Oj^{(k)})+ %\varepsilon 
\sum_{\substack{ 1 \le j \le N \\ j \ne k  }} \boldsymbol{C}^{(j)} \cdot \BCD^{(j)}(\Bx)  %\XI_j)
\\
&&- %\varepsilon^3 
\sum_{\substack{    1 \le j \le N \\   j \ne k }} (\X-\Oj^{(j)})\cdot T(\Oj^{(k)}, \Oj^{(j)}) \BCQ^{(j)}\boldsymbol{C}^{(j)}  %- \psi_k 
 \;, 
\label{R3energyest3}
\end{eqnarray}
for all $\Bx \in \GO_N$ and $k=1,\dots,N$. 
%The constant $\psi_k$ in \eq{R3energyest3} is chosen in such a way that 
%\beq
%\int_{B_{3 \Gve}^{(k)}} \Psi_k(\Bx) d \Bx = 0.
%\eequ{psi_k}
%For a given $k$, the 
Every function $\Psi_k$ satisfies
\begin{equation}\label{R3energyest4}
-\Delta \Psi_k(\X)=f(\X)\;, \quad \X \in \Omega_N\;,
\end{equation}
and since $\omega    \cap    \text{supp } f=\varnothing$, we %have 
see that $\Psi_k, ~k =1, \ldots, N,$ are harmonic in $\Go$. % \cap \GO_N$.
%Also, since 
Since the coefficients $\BC^{(j)}$ satisfy %the 
system \eq{alg1}, %on the boundary $\prt F^{(k)}$ 
we obtain %have
\begin{equation}\label{R3energyest5}
\Dn{\Psi_k}{}(\X)+ \Dn{\mathcal{R}_N}{}(\X)=0\;, \quad \X \in \partial %\omega_\varepsilon
F^{(k)}\;.
\end{equation}
%and $\Psi_k(\Bx) \to 0$ as $|\Bx| \to \infty.$ 
%Also it follows from the definition \eq{R3energyest3} that 
and according to \eq{rem2} the functions $\Psi_k$ have %a 
zero flux through the boundaries of small voids $%\Go_\Gve
F^{(k)}$, i.e. 
%%and the zero flux condition
\begin{equation}\label{R3energyest6}
\int_{\partial 
%\omega_\varepsilon
F^{(k)}} \Dn{\Psi_k}{}(\X)\, d\X=0\;, k=1, \dots, N\;.
\end{equation}

Next, we introduce smooth cutoff functions $$\chi_\Gve^{(k)}: \Bx \to \chi%_k(%\fr{
((\Bx - \BO^{(k)})/ %}{ 
\Gve %d
%}
), ~ k= 1, \ldots, N,$$ 
%in such a way that % $\chi_k(t)$ are smooth, 
%$$\chi_k\Big(\fr{\Bx - \BO^{(k)}}{\Gve %d
%}\Big) = 0 ~~\mbox{when}~ \Bx \in {\Bbb R}^3 \setminus \ov{B}_{%10 
%3 \Gve %d/4
%}^{(k)},$$ and
%$$\chi_k\Big(\fr{\Bx - \BO^{(k)}}{\Gve %d
%}\Big) = 1 ~~\mbox{when}~ \Bx \in  B_{%3 
%2 \Gve}^{(k)}.$$ 
%It is also assumed that all derivatives of $\chi_k(\fr{\Bx - \BO^{(k)}}{d})$ are equal to zero when
%$|\Bx- \BO^{(k)}| = d/4.$
equal to $1$ on $B_{2 \Gve}^{(k)}$ and vanishing outside $B_{3 \Gve}^{(k)}$. 
%It is assumed that $\chi_k(t) \in C_0^\infty(B_{3 %10 %1/4
%})$.
%We also use the notation $\chi^{(k)}_\Gve(\Bx) =  \chi%_k(%\fr{
%((\Bx - \BO^{(k)})/ %}{ 
%\Gve %d
%%}
%)$. 
Then %we note that  
by \eq{R3energyest5} we have  %\eq{R3energyest3} and \eq{alg1}%the function
\beq
\fr{\prt}{\prt n}\Big(\CR_N(\Bx) + \sum_{1 \leq k \leq N} \chi^{(k)}_\Gve(\Bx) %k\Big(%d^{-1} 
%(\Bx - \BO^{(k)})/\Gve \Big) 
\Psi_k(\Bx)\Big) = 0 ~~\mbox{on}~~ \prt %\Go_\Gve
F^{(j)}, ~ j = 1, \ldots, N.
\eequ{rem_1a}
%satisfies the homogeneous Neumann boundary conditions on $\prt \Go_\Gve^{(j)}, ~ j = 1, \ldots, N,$ and vanishes at infinity.

%Next, we introduce the \emph{relative capacitary potentials} $P_k$, $k=1, \dots, N$, which solve 
%\begin{equation}\label{R3energyest7}
%\left. \begin{array}{c}
%\Delta P_k(\X)=0\;, \quad \X \in B^{(k)}_{d/4} \backslash \bar{\omega}_\varepsilon^{(k)}\;,\\ \\
% P_k(\X)=1\;, \quad \X \in \partial \omega_\varepsilon^{(k)}\;,\\ \\
% P_k(\X)=0\;, \quad \text{ when }| \X-\Oj^{(k)}|=d/4\;, 
% \end{array}\right\}
% \end{equation}
% for $k=1, \dots, N$ and we extend the functions $P_k$, $k=1, \dots, N$ by zero outside $\overline{B^{(k)}_{d/4}}$. %In \cite{MMMeso}, it was shown that $P_k$ satisfies the estimate
% By the maximum principle 
% \begin{equation}\label{R3energyest8}
% |P_k(\X)| \le \text{const } \frac{\varepsilon}{|\X-\Oj^{(k)}|}\;, \text{for }\X \in B^{(k)}_{d/4} \backslash \overline{B^{(k)}_{3\varepsilon}}\;.
% \end{equation}
% %\begin{equation}\label{R3energyest9}
% %|\nabla P_k(\X)| \le \text{const } \frac{\varepsilon}{|\X-\Oj^{(k)}|^2}\;, \text{for }\X \in B^{(k)}_{d/4} \backslash \overline{B^{(k)}_{3\varepsilon}}\;.
%% \end{equation}
% %In parts $b)$ and $c)$ we use the notation 
% %\[ \BRN=B_R \backslash \overline{\cup_{j=1}^N \omega_\varepsilon^{(j)}}\;. \]
 \emph{c) %The energy of $\mathcal{R}_N$ versus %$P_k$ and 
 %$\Psi_k$.
 Estimate of the energy integral of  $\mathcal{R}_N$  in terms of  $\Psi_k$.}
 %We use the notation 
 %\[ \BRN=B_R \backslash \overline{\cup_{j=1}^N %\omega_\varepsilon
 %F^{(j)}}\; , \]
% where $B_R = \{\Bx: |\Bx| <R\}$, and  $R$ is sufficiently large. 
%% and %we 
% %derive an expression which allows us to estimate the energy of $\mathcal{R}_N$. % using the functions appearing in part $a)$ of the proof. 
 Integrating by parts in $\GO_N$ and using the definition of %the cut-off functions 
 $\chi^{(k)}_\Gve %k
 $, 
 %together with the harmonicity of $\mathcal{R}_N$,
  we write   the identity
  \begin{eqnarray} %uation}
   \int_{\GO_N %\BRN
   }\nabla \mathcal{R}_N
   %(\X) 
   \cdot \nabla \Big( \mathcal{R}_N
   %(\X)  
    + \sum_{1 \leq k \leq N} \chi^{(k)}_\Gve %k
    %\Big((\Bx - \BO^{(k)})/  \Gve %d
   %\Big) 
   \Psi_k
   %(\Bx) 
   \Big)\, d\X %= I_1 - I_2,
%   \nonumber \\
 % & = - \int_{\BRN}\mathcal{R}_N(\X)  \GD \Bigg( \mathcal{R}_N(\X)   + \sum_{1 \leq k \leq N} \chi_k\Big( (\Bx - \BO^{(k)})/d\Big) \Psi_k(\Bx) \Bigg)\, d\X %\nonumber  \\
 %  &&~~~ 
 %+ \int_{\prt B_R} \CR_N(\Bx) \fr{\prt}{\prt n} \CR_N(\Bx) d s_\X. & 
 %\label{rem_1}
  %\end{equation}
% where 
 %\beq
 %I_1 =  \int_{\prt B_R} \CR_N(\Bx) \fr{\prt}{\prt n} \CR_N(\Bx) d s_\X,
 %\eequ{rem_1A}
 %and 
 %\beq
 %I_2 
 = -  \int_{\GO_N %\BRN
 }\mathcal{R}_N
 %(\X) 
  \GD \Big( \mathcal{R}_N
  %(\X)   
  + \sum_{1 \leq k \leq N} \chi^{(k)}_\Gve %k\Big( (\Bx - \BO^{(k)})/ \Gve %  d
 %\Big) 
 \Psi_k
 %(\Bx) 
 \Big)\, d\X,
  %\eequ
  \label{rem_1B}
 \end{eqnarray}
 %Due to (\ref{R3formalgeq8}), for the first integral on the right-hand side of \eq{rem_1} %, due to (\ref{R3formalgeq8}) 
% we have
%\beq 
%%\Big|\int_{\partial B_R} \mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X\Big|
%|I_1|=O(R^{-1}),\eequ{rem_1b}
%whereas 
which is equivalent to 
 \begin{eqnarray}
   \int_{\GO_N 
   }\big| \nabla \mathcal{R}_N\big|^2 d\X + \sum_{1 \leq k \leq N}  \int_{B_{3 \Gve}^{(k)} \setminus \ov{F}^{(k)}
   }
  \nabla \mathcal{R}_N \cdot \nabla \big(  \chi^{(k)}_\Gve  
   \Psi_k
   \big)\, d\X = -  \sum_{1 \leq k \leq N} \int_{ B_{3 \Gve}^{(k)} \setminus \ov{F}^{(k)}  %\GO_N 
 }\mathcal{R}_N
  \GD \big(  \chi^{(k)}_\Gve  \Psi_k
 \big)\, d\X,
  \label{rem_1BB}
 \end{eqnarray}
since $\mathcal{R}_N$ is harmonic in $\Omega_N$.

%Let $\tilde{\CR}_N$ denote 
We preserve the notation $\CR_N$ for an extension of $\CR_N$ onto the union of voids $F^{(k)}$ with preservation of the class $W^{1,2}$. Such an extension can be constructed
by using only values of $\CR_N$ on the sets $B_{%4 
2 \Gve}^{(k)} \setminus \ov{F}^{(k)}$ in such a way that
\beq  
\| \Grad %\tilde
{\CR}_N \|_{L^2(B_{%4 
2 \Gve}^{(k)})} \leq \mbox{\rm const} \| \Grad \CR_N \|_{L^2(B_{%4 
2 \Gve}^{(k)} \setminus \ov{F}^{(k)})}.
\eequ{CN}
The above fact follows by dilation $\Bx \to \Bx / \Gve$ from the well-known extension theorem for domains with Lipschitz boundaries (see Section 3 of Chapter 6 in \cite{stein}). %, Section .....). 
We 
%choose the constant
%$\Gamma^{(k)}$ in \eq{rem_45} 
shall use the notation $\ov{\CR}^{(k)}$ for the mean value of $%\tilde
{\CR}_N$ on $B_{%10 
3 \Gve}^{(k)}$. 


%Since $\GD \CR_N(\Bx)= 0 $ on $\GO_N$,  
The % second 
integral  on the right-hand side of \eq{rem_1BB} can be written as
\begin{eqnarray}
%&&\int_{\BRN}\mathcal{R}_N(\X)  \GD \Big( \mathcal{R}_N(\X)   + \sum_{1 \leq k \leq N} \chi_k\Big(d^{-1} (\Bx - \BO^{(k)})\Big) \Psi_k(\Bx) \Big)\, d\X \nonumber \\
%&&%I_2 = 
-\sum_{1 \leq k \leq N}   \int_{B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)}} \CR_N
%(\X) 
\GD \big( \chi^{(k)}_\Gve %k\Big((\Bx - \BO^{(k)})/ \Gve %d
%\Big) 
\Psi_k
%(\Bx) 
\big)\, d\X
%\label{rem_2} \\
%&& 
= - \sum_{1 \leq k \leq N}    \int_{B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)}} (\CR_N%(\X)
- 
\ov{\CR}
%\Gamma
^{(k)}%_N
)  \GD \big( \chi^{(k)}_\Gve %k\Big( (\Bx - \BO^{(k)})/ \Gve %d
%\Big) 
\Psi_k
%(\Bx) 
\big)\, d\X, \label{rem_2}% \nonumber
\end{eqnarray}
%where $%\ov{\CR}
%\Gamma^{(k)}%_N
%$ is a constant to be defined later. %the average of $\CR_N$ over $B_{d/4}^{(k)} \setminus \ov{F%\Go
%}%_\Gve
%^{(k)}$. 
In the derivation of %the above equation 
\eq{rem_2} we have used that
\begin{eqnarray}
 &&\int_{B_{%10 
 3 \Gve %d/4
 }^{(k)} \setminus \ov{F %\Go
 }%_\Gve
 ^{(k)}}  \GD \Big( \chi^{(k)}_\Gve %k\Big( (\Bx - \BO^{(k)})/\Gve %d
 %\Big) 
 \Psi_k %(\Bx)
  \Big)\, d\X % \nonumber \\
 %&& 
 = \int_{\prt F %\Go_\Gve
 ^{(k)}} \fr{\prt   \Psi_k }{\prt n} 
 %(\Bx) 
  d S_\X = 0 \label{rem_3}
\end{eqnarray}
according to  \eq{R3energyest6} and  the definition of $\chi^{(k)}_\Gve %k
$.

%Taking the limit in \eq{rem_1}  as $R \to \infty$ and using \eq{rem_1b} and \eq{rem_2} we deduce
Owing to \eq{rem_1B%b
} and \eq{rem_2}, we can write 
\begin{eqnarray}
\| \Grad \CR_N \|^2_{L^2(\GO_N)} &&\leq  \GS_1 + \GS_2 , \label{rem_4}
\end{eqnarray} 
where
\beq
\GS_1 = \sum_{1 \leq k \leq N} \Big|  \int_{B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F% \Go
}%_\Gve
^{(k)}}  \Grad \CR_N
%(\Bx) 
\cdot \Grad  \big( \chi^{(k)}_\Gve %k\big( (\Bx - \BO^{(k)})/ \Gve %d
%\big) 
\Psi_k
%(\Bx) 
\big) d\X  \Big| ,
\eequ{rem_44}
and
\beq
\GS_2= \sum_{1 \leq k \leq N} \Big|  \int_{B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)}}  (\CR_N
%(\X)
- %\Gamma %
\ov{\CR}
^{(k)} )
%_N)
  \GD \big( \chi^{(k)}_\Gve %k\big( (\Bx - \BO^{(k)})/ \Gve %d
%\big)
( \Psi_k%(\Bx) 
- \ov{\Psi}_k  ) \big)\, d\X \Big| ,
\eequ{rem_45}
where 
%the constant 
$\ov{\Psi}_k$ is 
%chosen as the average 
the mean value of $\Psi_k$ over the ball $B_{3 \Gve}^{(k)}$.
Here, we have taken into account that by harmonicity of $\CR_N$,  \eq{rem2} and definition of $\chi_\Gve^{(k)}$
$$
\int_{B_{3 \Gve}^{(k)}\setminus \ov{F}^{(k)}} \GD \Big( \CR_N - \ov{\CR}^{(k)}\Big)
\chi^{(k)}_\Gve %k\Big(  \fr{\Bx - \BO^{(k)}}{\Gve} \Big) \Big)
d \Bx=\int_{B_{3 \Gve}^{(k)}} \GD %\Big(
\Big( \CR_N - \ov{\CR}^{(k)}\Big) \chi^{(k)}_\Gve %k\Big(  \fr{\Bx - \BO^{(k)}}{\Gve} \Big) \Big) 
d \Bx = 0 .
%$$
%\mbox{       and   }
%%$$
%\int_{B_{3 \Gve}^{(k)}\setminus \ov{F}^{(k)}} \CR_N
%%(\Bx) 
%\GD \chi^{(k)}_\Gve %k\Big(  \fr{\Bx - \BO^{(k)}}{\Gve} \Big) 
%d \Bx = 0,
$$
%where the last equality holds due to the fact that $\CR_N$ is harmonic in $B_{3 \Gve}^{(k)}\setminus \ov{F}^{(k)}$, and it
%satisfies \eq{rem2}. 


%Due to 
By the Cauchy inequality, the first sum in \eq{rem_4} allows for the estimate
\begin{eqnarray}
%\sum_{1 \leq k \leq N} \Big|  \int_{B_{d/4}^{(k)} \setminus \ov{\Go}_\Gve^{(k)}}  \Grad \CR_N(\Bx) \cdot \Grad  \big( \chi_k\big(d^{-1} (\Bx - \BO^{(k)})\big) \Psi_k(\Bx) \big) d\X  \Big| 
\GS_1 
%\leq
%\sum_{1 \leq k \leq N}  \Bigg( \int_{B_{%10 
%3 \Gve %d/4
%}^{(k)} \setminus \ov{F %\Go
%}%_\Gve
%^{(k)}}  |\Grad \CR_N
%%(\Bx)
%|^2 d\X  \Bigg)^{1/2}  % \nonumber \\
%%\times
%\Bigg( \int_{B_{%10
%3 \Gve %d/4
%}^{(k)} \setminus \ov{F  %\Go
%}%_\Gve
%^{(k)}}  \Big| \Grad  \big( \chi^{(k)}_\Gve %k\big( (\Bx - \BO^{(k)})/\Gve %d
%%\big) 
%\Psi_k
%%(\Bx) 
%\big) \Big|^2 d\X  \Bigg)^{1/2}   \nonumber \\
\leq \Big( \sum_{1 \leq k \leq N}  \|   \Grad \CR_N   \|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)})}    \Big)^{1/2} \Big( \sum_{1 \leq k \leq N}  \Big\|   \Grad  \big( \chi^{(k)}_\Gve %_k\big( (\Bx - \BO^{(k)})/ \Gve %d
%\big) 
\Psi_k
%(\Bx) 
\big)    \Big\|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)})}    \Big)^{1/2} \;.
\l{rem_55}
\end{eqnarray}
Furthermore, using the inequality 
\beq
 \sum_{1 \leq k \leq N}  \|   \Grad \CR_N   \|^2_{L^2(B_{3 %10 
 \Gve %d/4
 }^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)})}
\leq \|   \Grad \CR_N   \|_{L^2(\GO_N)}^2,
\eequ{rem_56}
together with \eq{rem_55}, we deduce
\begin{eqnarray}
\GS_1 
\leq \|   \Grad \CR_N   \|_{L^2(\GO_N)} \Big( \sum_{1 \leq k \leq N} \big\|   \Grad  \big( \chi^{(k)}_\Gve %k\big( (\Bx - \BO^{(k)})/ \Gve %d
%\big) 
\Psi_k %(\Bx) 
\big)    \big\|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F %\Go
}%_\Gve
^{(k)})}    \Big)^{1/2}. \label{rem_5}
\end{eqnarray} 
%In turn, with the use of the Poincar\'{e} inequality  the second sum in \eq{rem_4} can be estimated as follows

%Let $\tilde{\CR}_N$ denote an extension of $\CR_N$ onto the union of voids $F^{(k)}$ with preservation of the class $W_2^1$. Such an extension can be constructed
%by using only values of $\CR_N$ on the sets $B_{%4 
%2 \Gve}^{(k)} \setminus \ov{F}^{(k)}$ in such a way that
%\beq  
%\| \Grad \tilde{\CR}_N \|_{L_2(B_{%4 
%2 \Gve}^{(k)})} \leq \mbox{\rm const} \| \Grad \CR_R \|_{L_2(B_{%4 
%2 \Gve}^{(k)} \setminus \ov{F}^{(k)})}.
%\eequ{CN}
%The above fact follows by dilation $\Bx \to \Bx / \Gve$ from the well-known extension theorem for domains with Lipschitz boundaries (see \cite{stein}, Section .....). 
%
%We choose the constant
%$\Gamma^{(k)}$ in \eq{rem_45} as the mean value of $\tilde{\CR}_N$ on $B_{%10 
%3 \Gve}$. 

Similarly to \eq{rem_55}, the second sum in \eq{rem_4} can be estimated as  %follows
\begin{equation}
%&& \sum_{1 \leq k \leq N} \Big|  \int_{B_{d/4}^{(k)} \setminus \ov{\Go}_\Gve^{(k)}}  (\CR_N(\X)-\ov{\CR}^{(k)}_N)  \GD \big( \chi_k\big(d^{-1} (\Bx - \BO^{(k)})\big) \Psi_k(\Bx) \big)\, d\X \Big| \nonumber \\
\GS_2  \leq  \sum_{1 \leq k \leq N}  \Big( \int_{B_{%10
3 \Gve %d/4
}^{(k)} %\setminus \ov{F %\Go
%}%_\Gve
%^{(k)}
}  (%\tilde
{\CR}_N %(\X)
-   \ov{\CR}
%\Gamma
^{(k)}%_N
)^2 d \X \Big)^{1/2}
 \Big( \int_{B_{%10 
 3 \Gve %d/4
 }^{(k)} \setminus \ov{F %\Go
 }%_\Gve
 ^{(k)}}     \big( \GD ( \chi^{(k)}_\Gve %k\big( (\Bx - \BO^{(k)})/  \Gve %d
 %\big) 
 ( \Psi_k
 %(\Bx) 
 - \ov{\Psi}_k ) ) \big)^2\, d\X   \Big)^{1/2} .  %\nonumber \\
\label{rem_66}
 \end{equation}
% Then using the
% and by 
By the Poincar\'{e} inequality for the ball $B^{(k)}_{%10 
 3 \Gve}$ %, together with \eq{rem_56}, 
 \beq
%\|\Psi_k - \ov{\Psi}_k \|_{L_2(B^{(k)}_{3 \Gve})}^2 \leq \mbox{\rm const  } \Gve^2 \| \Grad \Psi_k \|_{L_2(B^{(k)}_{3 \Gve})}^2
\|\CR_N - \ov{\CR}^{(k)} \|_{L^2(B^{(k)}_{3 \Gve})}^2 \leq \mbox{\rm const  } \Gve^2 \| \Grad \CR_N \|_{L^2(B^{(k)}_{3 \Gve})}^2
\eequ{Psi_k_ball} 
 we obtain
% \begin{eqnarray}
 $$
 \GS_2 \leq \mbox{const}~ %d
 \Gve  ~\Big( \sum_{1 \leq k \leq N}  \|   \Grad %\tilde
 {\CR}_N   \|^2_{L^2(B_{%10 
 3 \Gve %d/4
 }^{(k)}) %\setminus \ov{F %\Go
% }%_\Gve
% ^{(k)})
}    \Big)^{1/2} \Big( \sum_{1 \leq k \leq N}  \int_{B_{%10 
3 \Gve %d/4
}^{(k)} \setminus \ov{F  %\Go
 }% _\Gve
 ^{(k)}}     \big( \GD ( \chi^{(k)}_\Gve %k\big((\Bx - \BO^{(k)})/  \Gve %d 
 %\big) 
 ( \Psi_k %(\Bx) 
 - \ov{\Psi}_k ) ) \big)^2\, d\X \Big)^{1/2},
 $$ %\nonumber \\
  which does not exceed
 \begin{eqnarray}
 &%\leq
 & \mbox{const}~ \Gve %d 
 ~\|   \Grad \CR_N   \|_{L^2(\GO_N)}    \Big( \sum_{1 \leq k \leq N}  \int_{B_{%10 
 3 \Gve %d/4
 }^{(k)} \setminus \ov{F %\Go
 }%_\Gve
 ^{(k)}}     \big( \GD \big( \chi^{(k)}_\Gve %k\big((\Bx - \BO^{(k)})/ \Gve \big) 
 ( \Psi_k
 %(\Bx) 
 - \ov{\Psi}_k ) \big) \big)^2\, d\X \Big)^{1/2}  , \label{rem_6}
\end{eqnarray} 
because of \eq{CN}. 
Combining \eq{rem_4}--\eq{rem_6} and dividing both sides of \eq{rem_4} by $\| \Grad \CR_N \|_{L^2(\GO_N)}$  we arrive at
\begin{eqnarray}
 \| \Grad \CR_N \|_{L^2(\GO_N)} &&\leq \Big( \sum_{1 \leq k \leq N}  \Big\|   \Grad  \big( \chi^{(k)}_\Gve %k\big( (\Bx - \BO^{(k)})/ \Gve %d 
% \big) 
( \Psi_k%(\Bx) 
- \ov{\Psi}_k  ) \big)   \Big\|^2_{L^2(B_{%10 
 3 \Gve %d/4
 }^{(k)} %\setminus \ov{
 %F %\Go
 %}_\Gve
 %^{(k)}
 )}    \Big)^{1/2} \nonumber \\
&& + \mbox{const} ~ \Gve %d 
~  \Big( \sum_{1 \leq k \leq N}  \int_{B_{%10 
3 \Gve %d/4
}^{(k)} %\setminus \ov{F %\Go
%}%_\Gve
%^{(k)}
}     \big\{ (\Psi_k
%(\Bx)
-\ov{\Psi}_k) \GD %\Big( 
\chi^{(k)}_\Gve %k \big( (\Bx - \BO^{(k)})/ \Gve %d  
%\big) 
%\Big) 
%\nonumber \\
%&&  
+ 2 \Grad %\bigg( 
\chi^{(k)}_\Gve %k \big( (\Bx - \BO^{(k)}) /  \Gve %d 
%\big) 
%\bigg) 
\cdot \Grad \Psi_k
%(\Bx) 
%\bigg) 
\big\}^2\, d\X \Big)^{1/2}, \label{rem_7}
\end{eqnarray}
%where $\ov{\Psi}_k$ denotes the average of $\Psi_k$ over the ball $B_{3 \Gve}^{(k)}$. In turn, the estimate \eq{rem_7} 
which leads to
\begin{eqnarray}
&& \| \Grad \CR_N \|^2_{L^2(\GO_N)} \leq \mbox{const} \sum_{1 \leq k \leq N} \Big( \|   \Grad \Psi_k \|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} %\setminus \ov{F %\Go
%}%_\Gve
%^{(k)}
)
}  + \Gve %d
^{-2} \|   \Psi_k - \ov{\Psi}_k\|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} %\setminus \ov{F %\Go
%}%_\Gve
%^{(k)}
)
}    \Big). \label{Psi_k_ball_1}
\end{eqnarray}
%Since $\Psi_k$ has the zero average over $B_{3 \Gve}^{(k)}$ (see \eq{psi_k}), we apply 
Applying the Poincar\'{e} inequality (see \eq{Psi_k_ball}) for $\Psi_k$ in the ball $B_{3 \Gve}^{(k)}$ and using \eq{Psi_k_ball_1},  we deduce
%\beq
%\|\Psi_k - \ov{\Psi}_k \|_{L_2(B^{(k)}_{3 \Gve})}^2 \leq \mbox{\rm const  } \Gve^2 \| \Grad \Psi_k \|_{L_2(B^{(k)}_{3 \Gve})}^2
%\eequ{Psi_k_ball} 
%
%The estimates \eq{Psi_k_ball_1} and \eq{Psi_k_ball} yield
\begin{eqnarray}
&& \| \Grad \CR_N \|^2_{L^2(\GO_N)} \leq \mbox{const} \sum_{1 \leq k \leq N} 
\|   \Grad \Psi_k \|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} %\setminus \ov{F %\Go
%}%_\Gve
%^{(k)}
)
}  . \label{Psi_k_ball_2}
\end{eqnarray}
 
 
% \begin{eqnarray*}
% \int_{\BRN}\nabla \mathcal{R}_N(\X) \cdot \nabla \mathcal{R}_N(\X)\, d\X&=& \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X-\sum_{k=1}^N \int_{\partial \omega_\varepsilon^{(k)}} \mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X\\
 %&=& \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X+\sum_{k=1}^N \int_{\partial \omega_\varepsilon^{(k)}} \mathcal{R}_N(\X)P_k(\X) \Dn{\Psi_k}{}(\X)\, ds_\X\;.
 %\end{eqnarray*}
 %since $P_k=1$ on $\partial \omega_\varepsilon^{(k)}$.
% %Here in 
 %In the last equality, we %also 
% employed (\ref{R3energyest5}). From this, since $P_k(\X)=0$ outside $B^{(k)}_{d/4}$ and $\Psi_k(\X)$ satisfies  (\ref{R3energyest4}) in $\BRN$, we deduce % the divergence theorem yields
 %\begin{eqnarray*}
% \| \nabla \mathcal{R}_N\|^2_{L_2(\BRN)}&=& \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X +\sum^N_{k=1} \int_{\BRN} \mathcal{R}_N (\X)P_k(\X) f(\X)\, d\X\\
 %&&-\sum^N_{k=1} \int_{\BRN} \nabla (\mathcal{R}_N(\X) P_k(\X))\cdot \nabla \Psi_k(\X)\, d\X\;.
% \end{eqnarray*}
% The second integral %in 
% on the right-hand side is zero owing to the fact that $\text{supp } P_k \cap \text{supp }f=\varnothing$.
% Hence
% \begin{equation}\label{R3energyest10}
 %\| \nabla \mathcal{R}_N\|^2_{L_2(\BRN)}= \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X 
% -\sum^N_{k=1} \int_{\BRN} \nabla (\mathcal{R}_N(\X) P_k(\X))\cdot \nabla \Psi_k(\X)\, d\X\;.
% \end{equation}
%We set 
%\[\widehat{\mathcal{R}_N}=(\text{meas}_3 (B_{R, N}))^{-1} \int_{B_{R, N}} \mathcal{R}_N(\X)\, d\X\;,\]
%where $\text{meas}_3(\BRN)$ is the volume of $\BRN$. Then, we can %re
%write (\ref{R3energyest10}) as
%  \begin{eqnarray*}
% \| \nabla \mathcal{R}_N\|^2_{L_2(\BRN)}&=& \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X-\sum^N_{k=1} \int_{\BRN} P_k(\X) \nabla \mathcal{R}_N(\X)\cdot \nabla \Psi_k(\X)\, d\X\\
% &&-\sum_{k=1}^N\int_{\BRN}(\mathcal{R}_N(\X)-\widehat{\mathcal{R}_N}) \nabla P_k(\X) \cdot \nabla \Psi_k(\X)\, d\X\\
% &&-\sum^N_{k=1}\widehat{\mathcal{R}_N} \int_{\BRN}\nabla P_k(\X)\cdot \nabla \Psi_k(\X)\,d\X\;.
% \end{eqnarray*}
%% The last sum, by Green's first identity, is equivalent to
 %Integration by parts in the last sum gives
% \begin{eqnarray}\label{R3energyest11}\nonumber
% -%\sum^N_{k=1} 
% \widehat{\mathcal{R}_N} \int_{\BRN} \nabla P_k(\X) \cdot \nabla \Psi_k(\X)\, d\X&=& %\sum^N_{k=1} 
% \widehat{\mathcal{R}_N} \left\{-\int_{\BRN} P_k(\X)f(\X)\, d\X+\int_{\partial \omega_\varepsilon^{(k)}} \Dn{\Psi_k}{}(\X)\, ds_\X\right\}\\
% &=& %\sum^N_{k=1}
% \widehat{\mathcal{R}_N} \int_{\partial \omega_\varepsilon^{(k)}} \Dn{\Psi_k}{}\, d\X=0\;,
% \end{eqnarray}
% where the zero flux condition (\ref{R3energyest6}) has been used. Thus, we have  arrived at
% \begin{eqnarray*}
 %\| \nabla \mathcal{R}_N\|^2_{L_2(\BRN)}&=& \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X\\ 
% &&-\sum^N_{k=1} \int_{\BRN} P_k(\X)\nabla \mathcal{R}_N (\X)\cdot \nabla \Psi_k(\X)\, d\X\\
% &&-\sum_{k=1}^N\int_{\BRN}(\mathcal{R}_N(\X)-\widehat{\mathcal{R}_N}) \nabla P_k(\X) \cdot \nabla \Psi_k(\X)\,d\X\;.
 %\end{eqnarray*}
 %By the Cauchy inequality, one has
% \begin{eqnarray*}
 %\| \nabla \mathcal{R}_N\|^2_{L_2(\BRN)}&\le& \Big|\int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, d s_\X \Big|\\
% &&+\| \nabla\mathcal{R}_N\|_{L_2(\BRN)}\Big\|\sum^N_{k=1}    P_k \nabla \Psi_k\Big\|_{L_2(\BRN)}\\
% &&+\|\mathcal{R}_N(\X)-\widehat{\mathcal{R}_N}\|_{L_2(\BRN)}\Big\|\sum_{k=1}^N \nabla P_k \cdot \nabla \Psi_k\Big\|_{L_2(\BRN)}\;.
 %\end{eqnarray*}
 %Then, Poincare's inequality gives 
 %\begin{eqnarray}\label{R3energyest12}
% \| \nabla \mathcal{R}_N\|^2_{L_2(\BRN)}&\le&\Big| \int_{\partial B_R}\mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X\Big| \nonumber\\
%+  && \text{const } ~\| \nabla \mathcal{R}_N\|_{L_2(\BRN)} \Big( \Big\|\sum^N_{k=1}    P_k \nabla \Psi_k\Big\|_{L_2(\BRN)}    %\nonumber\\
% %&&+\text{const }\| \nabla \mathcal{R}_N\|_{L_2(\BRN)}
% + \Big\|\sum_{k=1}^N \nabla P_k \cdot \nabla \Psi_k\Big\|_{L_2(\BRN)} \Big) \;.
 %\end{eqnarray}
%where here $\text{const}$ is the constant apprearing in the  inequality mentioned.
%
%As a result of the condition (\ref{R3formalgeq8}) for $\mathcal{R}_N$, we have
%\[ \Big|\int_{\partial B_R} \mathcal{R}_N(\X) \Dn{\mathcal{R}_N}{}(\X)\, ds_\X\Big|=O(R^{-1})\]
%and so passing to the limit as $R \to \infty$ in (\ref{R3energyest12}) we derive the inequality
%\[ \| \nabla \mathcal{R}_N\|^2_{L_2(\Omega_N)}\le \text{const }\Big(\Big\|\sum_{k=1}^N \nabla P_k \cdot \nabla \Psi_k\Big\|^2_{L_2(\Omega_N)}  + \Big\|\sum^N_{k=1}    P_k \nabla \Psi_k\Big\|^2_{L_2(\Omega_N)} \Big)\;.\]

\emph{d) %The 
Final energy estimate. }Here we prove the inequality \eq{introeq2}. %(\ref{R3energyest2}). 
 Using %the 
 definition \eq{R3energyest3} of 
%Due to the supports of the functions 
$\Psi_k$, $k=1, \dots, N$, we can replace  the preceding inequality by
%can be replaced by
%\begin{equation}\label{R3ineq}
%\| \nabla \mathcal{R}_N\|^2_{L_2(\Omega_N)}\le \text{const }\Big(   \sum_{k=1}^N \|\nabla P_k \cdot \nabla \Psi_k\|^2_{L_2(B^{(k)}_{d/4} \backslash \overline{\omega_\varepsilon^{(k)}})}   + \sum^N_{k=1}  \| P_k \nabla \Psi_k\|^2_{L_2(B^{(k)}_{d/4} \backslash \overline{\omega_\varepsilon^{(k)}})} \Big)\;.
%\end{equation}
%Then from this we can deduce
%obtain the inequality
\begin{equation}\label{R3energyest12a}
\| \nabla \mathcal{R}_N\|^2_{L^2(\Omega_N)}\le \text{const } \big\{ \mathcal{K}+\mathcal{L} %+ \mathcal{S}+\mathcal{T} 
\big\}\;,
\end{equation}
where 
\begin{equation}\label{R3energyest13}
\begin{array}{l}\displaystyle{ \mathcal{K}=\sum_{1\le k\le N} \| \nabla v%_f 
(\cdot %\Bx
)- \nabla v%_f
(\Oj^{(k)})\|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} % \backslash \overline{F %\omega_\varepsilon
%^{(k)}}
)}\;,}\\
\\
\displaystyle{\mathcal{L}= %\varepsilon^2
\sum_{1 \le k \le N} \Big\| \sum_{\substack{j \ne k \\ 1 \le j \le N}}  \Big[\nabla \Big(\boldsymbol{C}^{(j)} \cdot \BCD^{(j)}(\cdot %\Bx %XI_j
) \Big)- %\varepsilon^2 
T(\Oj^{(k)}, \Oj^{(j)})\BCQ^{(j)}\boldsymbol{C}^{(j)} \Big] \Big\|^2_{L^2(B_{%10 
3 \Gve %d/4
}^{(k)} %\backslash \overline{F %\omega_\varepsilon
%^{(k)}}
)}.}
%\\ \\
%\displaystyle{\mathcal{S}= %d
%\Gve^{-2}\sum_{k=1}^N \|  v_f(\X) - v_f(\BO^{(k)})-(\Bx-\BO^{(k)}) \cdot \nabla v_f(\Oj^{(k)}))\|^2_{L_2(B_{10 \Gve %d/4
%} \backslash \overline{F %\omega_\varepsilon
%^{(k)}})},}\\ \\
%\displaystyle{\mathcal{T}= %\varepsilon^2 
%%d
%\Gve^{-2}
%\sum_{k=1}^N \Big\| \sum_{\substack{j \ne k\\ 1\le j \le N}} \Big[ \boldsymbol{C}^{(j)} \cdot \BCD^{(j)}(\XI_j))+\varepsilon^2  %(\Bx-\BO^{(k)}) \cdot T(\Oj^{(k)}, \Oj^{(j)})\BCQ^{(j)}\boldsymbol{C}^{(j)}
%\Big] \Big\|^2_{L_2(B_{10 \Gve %d/4
%}^{(k)} \backslash \overline{F %\omega_\varepsilon
%^{(k)}})}.}
\end{array} 
\end{equation}
%also $\mathcal{K}^{(2)}$ through to $\mathcal{T}^{(2)}$ are obtained by replacing $B_{3\varepsilon}^{(k)} \backslash \overline{\omega^{(k)}_\varepsilon}$ by $B_{d/4}^{(k)} \backslash \overline{B_{3\varepsilon}^{(k)}}$ in $\mathcal{K}^{(1)}$ through to $\mathcal{T}^{(1)}$, respectively.

The estimate for $\CK$ %and $\CS$ are 
is straightforward and %they 
it follows by Taylor's expansions of $v$ %_f$ 
in the vicinity of $\BO^{(k)}$,  %, ~ k = 1, \ldots, N$:
\beq
\CK % + \CS 
\leq \text{const }  \Gve^5 d^{-3}  \max_{\Bx \in \ov{\Go}, 1 \le i, j\le 3} \Big|\frac{\partial^2 v%_f
}{\partial x_i \partial x_j}\Big|^2. %~~\mbox{and}~~\CS \leq \text{const }  d^2  \max_{\Bx \in \Go, 1 \le i, j\le 3} \Big|\frac{\partial^2 v_f}{\partial x_i \partial x_j}\Big|^2.
\eequ{rem_8}
Since $v$ %_f$ 
is harmonic %on 
in a neighbourhood of $\ov{\Go}$, we obtain by the 
%generalized mean value theorem (see, for example, \cite{Mikhlin}) 
local regularity property of harmonic functions that
%
%
%The right-hand side in \eq{rem_8} can be estimated further in terms of $v_f$. We will need the averaging function $W_h(|\Bx - \By|)$ (see, for example, \cite{Mikhlin}) defined by
%$$
%W_h(r) = \left\{ \begin{array}{cc}
%\beta^{-1} ~\exp\{ -h^2 /(h^2-r^2)\} , & \mbox{when  } r < h,   \\
%0, & \mbox{when  } r \geq h,
%\end{array} \right. 
%$$
%where
%$$
%\Gb = 4 \pi h^3 \int_{0}^1 t^2 \exp\big(-1/(1-t^2)\big) dt.
%$$
%This function $W_h$ is infinitely differentiable and possesses the following properties:
%\begin{itemize}
%\item[(a)] $W_h(r) > 0$ when $r < h$, and $W_h(r) = 0$, together with all its derivatives, when $r \geq h$,
%\item[(b)] $\int_{| \Bx - \By  | < h} W_h(| \Bx - \By  |)  d \Bx =  \int_{| \Bx - \By  | < h} W_h(| \Bx - \By  |)  d \By = 1.$
%\end{itemize}
%
%For a given $\Bx \in \Go$, the function $v_f$ as well as $\frac{\partial^2 v_f}{\partial x_i \partial x_j}$ are harmonic in $B_h(\Bx) = \{ \By : |\Bx - \By| < h\},$ and the following representation holds
%%\beq
%$
%\frac{\partial^2 v_f (\Bx)}{\partial x_i \partial x_j} = \int_{B_h(\Bx)} \frac{\partial^2 v_f(\By)}{\partial y_i \partial y_j} W_h(|  \Bx - \By |) d \By.
%%\eequ{W_rem}
%$
%Then % the 
%integration by parts gives 
%\beq
%\frac{\partial^2 v_f (\Bx)}{\partial x_i \partial x_j}  = \int_{B_h(\Bx)}  v_f(\By)\frac{\partial^2 W_h(|  \Bx - \By |) }{\partial y_i \partial y_j} d  \By,
%\eequ{W_rem1}
%which leads to 
%\beq
%\Big| \frac{\partial^2 v_f (\Bx)}{\partial x_i \partial x_j} \Big| \leq \Big(  \int_{B_h(\Bx)} \big( v_f(\By)\Big)^2 d \By  \Big)^{1/2} \Big(  \int_{B_h(\Bx)} \Big(   \frac{\partial^2 W_h(|  \Bx - \By |) }{\partial y_i \partial y_j}  \Big)^2 d \By  %\Big)^{1/2} \leq \mbox{const  } \|v_f \|_{L_2(\Go_h)},
%\eequ{W_rem2}
%where the constant on the right-hand side of \eq{W_rem2} is independent of $\Gve$ and $d$, and the extended set $\Go_h$ is defined in \eq{om_h}. Hence, \eq{rem_8} and \eq{W_rem2} yield
\beq
\CK  %+ \CS 
\leq \text{const } \Gve^5 d^{-3}  \big\| \Grad v%_f 
\big\|^2_{L^2(  {\Bbb R}^3 ) %\Go_h)
}. %~~\mbox{and}~~\CS \leq \text{const }  d^2  \max_{\Bx \in \Go, 1 \le i, j\le 3} \Big|\frac{\partial^2 v_f}{\partial x_i \partial x_j}\Big|^2.
\eequ{rem_88}


To estimate $\CL$,  
%and $\CT$ 
we use Lemma \ref{Djasymp} on the asymptotics of the dipole fields together with the definition \eq{defT} of the matrix function $T$, which  lead to 
 \begin{equation}\label{R3energyest14}
 |\nabla(\boldsymbol{C}^{(j)} \cdot \BCD^{(j)}(\Bx))-  T(\Oj^{(k)}, \Oj^{(j)})\BCQ^{(j)} \boldsymbol{C}^{(j)}| \le \text{const }\varepsilon^4|\boldsymbol{C}^{(j)}| |\X-\Oj^{(j)}|^{-4}\;, %\text{ for } \X \in B^{(k)}_{d/4}\;,
 \end{equation}
% and
 % \begin{equation}\label{R3energyest14a}
 %|\boldsymbol{C}^{(j)} \cdot \BCD^{(j)}(\XI_j)+ (\Bx - \BO^{(j)}) \cdot \BT(\Oj^{(k)}, \Oj^{(j)})\BCQ^{(j)} \boldsymbol{C}^{(j)}| \le %\text{const }\varepsilon^4|\boldsymbol{C}^{(j)}| |\X-\Oj^{(j)}|^{-3}\;, %\text{ for } \X \in B^{(k)}_{d/4}\;,
 %\end{equation}
 for $ \X \in B^{(k)}_{%10 
 3 \Gve %d/4
 }.$ %Hence, 
 Now, it follows from \eq{R3energyest13} and \eq{R3energyest14} %, \eq{R3energyest14a} 
 that
\begin{eqnarray}
% \mathcal{L} &\le& \text{const } \varepsilon^8 \sum^N_{j=1} |\boldsymbol{C}^{(j)}|^2 \sum_{\substack{j \ne k\\ 1 \le k \le N}}%\int_{B^{(k)}_{10 \Gve %d/4
% } \backslash \overline{F %\omega_\varepsilon
% ^{(k)}}}  \fr{d\X}{ |\X-\Oj^{(j)}|^{8}}\, 
 %\le \text{const } \varepsilon^8 \sum^N_{j=1} |\boldsymbol{C}^{(j)}|^2 \int_{\{\Bx \in \Go, |\Bx - \BO^{(j)}| > d/4\}}\fr{d \Bx}{|\Bx-
 %\Oj^{(j)}|^{8}} \nonumber \\
 %%\end{eqnarray*}
% %Approximating the above double sum by a Riemann integral we have
%&\le& \text{const } \varepsilon^8
%d^{-5}
%%{-6}
%% \int_{\omega} 
%\sum_{1 \leq j \leq N} |\boldsymbol{C}^{(j)}|^2  \;, \label{rem_9}
\mathcal{L} &\le& \text{const } \varepsilon^8 \sum^N_{k=1} \int_{B_{3 \Gve}^{(k)}} 
\Big(   \sum_{1 \leq j \leq N, j \neq k} \fr{| \BC^{(j)} |}{|\Bx - \BO^{(j)}|^4} \Big)^2 d \Bx, \label{rem_9}
\end{eqnarray}
and by the Cauchy inequality % it
the right-hand side  does not exceed
\begin{eqnarray}
%{\small 
&\mbox{const  }& \Gve^8 \sum_{p=1}^N |\BC^{(p)}|^2 \sum_{k=1}^N \sum_{1 \leq j \leq N, j \neq k} \int_{B_{3 \Gve}^{(k)}}  \fr{d \Bx}{|\Bx - \BO^{(j)}|^8 } \leq \mbox{const  } \Gve^{11}\sum_{p=1}^N |\BC^{(p)}|^2 \sum_{k=1}^N \sum_{1 \leq j \leq N, j \neq k} 
 \fr{1 %d \Bx
 }{|\BO^{(k)} - \BO^{(j)}|^8 } %} 
 \nonumber \\
 &&\leq  \mbox{const  } \fr{\Gve^{11}}{d^6} \sum_{p=1}^N |\BC^{(p)}|^2 
 \int\int_{\{\omega \times \omega:  |\BX - \BY| > d\}} \fr{d \BX d \BY}{|\BX - \BY|^8} \leq \mbox{const  } \fr{\Gve^{11}}{d^8} \sum_{p=1}^N |\BC^{(p)}|^2 . \label{rem_99}
 \end{eqnarray}

%and
%\begin{eqnarray}
 %\mathcal{T} &\le& \text{const } \varepsilon^6 %8 d^{-2} 
 %\sum^N_{j=1} |\boldsymbol{C}^{(j)}|^2 \sum_{\substack{j \ne k\\ 1 \le k \le N}}\int_{B^{(k)}_{10 \Gve %d/4
 %} \backslash \overline{F %\omega_\varepsilon
 %^{(k)}}}  \fr{d\X}{ |\X-\Oj^{(j)}|^{6}}\, 
%\nonumber \\
% %\end{eqnarray*}
% %Approximating the above double sum by a Riemann integral we have
%& \le& \text{const } \varepsilon^6 %8 d^{-2}
%\sum^N_{j=1} |\boldsymbol{C}^{(j)}|^2 \int_{\{\Bx \in \Go,  |\Bx - \BO^{(j) \}}| > d/4\}}\fr{d \Bx}{|\Bx-\Oj^{(j)}|^{6}} \le \text{const } %\varepsilon^ 6 %8
%d^{- 3} %5}
%%{-6}
%% \int_{\omega} 
%\sum_{1 \leq j \leq N} |\boldsymbol{C}^{(j)}|^2  \;. \label{rem_10}
%\end{eqnarray}
Since the eigenvalues of the matrix $-\BQ$ satisfy the constraint \eq{Gl_min},  we can apply Corollary \ref{coro1_alg} and  use
 the 
estimate \eq{alg12} for the %expressions on the 
right-hand side of \eq{rem_99} %. % and \eq{rem_10}.
%Thus, we 
to obtain % of  together with \eq{rem_9} and \eq{rem_10} we deduce
\beq
\CL %+ \CT 
\leq \mbox{const}~ \Gve^{11} %8 
d^{-11}%8} 
\|\Grad v%_f
\|^2_{L^2(\Go)}.
\eequ{rem_11}
Combining \eq{R3energyest12a}, \eq{rem_88} and \eq{rem_11},  we arrive at \eq{introeq2} %\eq{R3energyest2} 
 and complete the proof. 
$\Box$
%\end{proof}

==> Mesoscale pdf/alg_sys_m_v1.tex <==
%\documentclass[11pt]{report}
%\usepackage{graphics}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{enumerate}
%\usepackage{mathrsfs}
%\usepackage[dvips]{graphicx}
%\usepackage{psfrag}
%\input macroarx
%\begin{document}

\section{\bf %The a
Algebraic system in the case $\GO = {\Bbb R}^3$} \label{alg_syst}

The algebraic system for the coefficients $\BC^{(j)}$ %has the form
can be written in the form 
\beq
\BC + %\Gve^3 
\BCS \BQ \BC = - \BGT, %_f,
\eequ{alg1}
where 
$$
\BC = ( (\BC^{(1)})^T, \ldots, (\BC^{(N)})^T )^T, ~~ \BGT%_f
 = ((\Grad v%_f
 (\BO^{(1)}))^T, \ldots , (\Grad v%_f
 (\BO^{(N)}))^T )^T,
$$
are vectors of the dimension $3N$, and 
\begin{eqnarray}
\BCS&&=[\CS_{ij}]_{i, j=1}^N, ~ 
\CS_{ij}=\left\{\begin{array}{ll}\displaystyle{(\nabla_{\Bz} \otimes \nabla_{\Bw})\left(\frac{1}{4\pi|\Bz-\Bw|}\right)\Big|_{\substack{\Bz=\BO^{(i)}\\ \Bw=\BO^{(j)}}}} & \quad \text{ if } i \ne j\\
& \\
0I_3 %\BI_3
&\quad \text{otherwise} , \end{array}  \right.  \label{alg2} \\
 \quad \mathbf{Q}&&=\mbox{diag}\{\BCQ^{(1)}, \dots, \BCQ^{(N)}\}\; ~~\mbox{is negative definite}.  \label{alg3}
\end{eqnarray}
These are $3N \times 3N$ matrices whose entries are $3\times 3$ blocks. The notation in \eq{alg2} %means that 
is interpreted as 
$$\CS_{ij} = \left\{\fr{1}{4 \pi}\fr{\prt}{\prt z_q}\Big(  \fr{z_r - O_r^{(j)}}{| \Bz - \BO^{(j)} |^3}\Big)\Big|_{\Bz=\BO^{(i)}}\right\}^3_{q, r=1}
~\mbox{ when  } i\neq j.$$

We %shall also 
use the piecewise constant vector function
\beq
\BGX(\Bx) = \left\{  \begin{array}{cc}
\BCQ^{(j)} \BC^{(j)}, ~~\mbox{when} ~~ \Bx \in \ov{B}_{d/4}^{(j)}, ~ j = 1, \ldots, N, \\
\\
0, ~~~\mbox{otherwise}, \end{array} \right.
\eequ{alg3a}
where $B_r^{(j)} = \{\Bx: |\Bx - \BO^{(j)}| < r \}.$

%{\bf Theorem 1.} 
\begin{thm}   \label{thm1_alg} 
%{\em 
Assume that $%\Gve
 \Gl_{max} < \emph{\text{const }} d^3$, where $\Gl_{max}$ is the largest eigenvalue of the positive definite matrix $-\BQ$ and the constant is independent of $d$. Then the algebraic system 
{\rm \eq{alg1}} is solvable and the vector coefficients $\BC^{(j)}$ satisfy the estimate %}
\beq
\sum_{j=1}^N | (\BC^{(j)})^T \BCQ^{(j)} \BC^{(j)} | \leq (1- \emph{\text{const }}\fr{%\Gve^3
\Gl_{max} }{ d^3}  )^{-2} \sum_{j=1}^N |(\Grad v%_f
(\BO^{(j)}))^T \BCQ^{(j)} \Grad v%_f
(\BO^{(j)})|.
\eequ{alg4}
\end{thm}

%\newpage

We %will 
%need 
consider the scalar product of \eq{alg1} and the vector $\BQ \BC$:
\beq
\langle \BC, \BQ \BC \rangle + % \Gve^3 
\langle \BCS \BQ \BC, \BQ \BC \rangle = -\langle \BGT,%_f, 
\BQ \BC \rangle.
\eequ{alg6}
Prior to the proof of %the 
Theorem we formulate and prove the following identity.


%{\bf Lemma 1.} 
\begin{lem} \label{lem1_alg}
 %{\em 
 a)
 The scalar product $\langle   \BCS \BQ \BC, \BQ \BC  \rangle $ admits the representation  %}
\begin{eqnarray}
\langle   \BCS \BQ \BC, \BQ \BC  \rangle &&= \fr{  576%768
}{\pi^3 %2 
d^6} \int_{{\Bbb R}^3}  \int_{{\Bbb R}^3} \fr{1}{| \BX - \BY  |} (\Grad \cdot \BGX(\BX))  (\Grad \cdot \BGX(\BY)) d \BY  d \BX \nonumber \\
&& - \fr{16}{ \pi d^3}
\sum_{j=1}^N   | \BCQ^{(j)}  \BC^{(j)} |^2.
\label{alg5m}
\end{eqnarray}

b) The following estimate holds
\[|\langle \BCS \BQ \BC, \BQ \BC\rangle| \le \text{\emph{const }}d^{-3}\, \sum_{1 \le j  \le N}|\BQ^{(j)} \BC^{(j)}|^2\;,\]
where the constant in the right-hand side does not depend on $d$.
\end{lem}


{\bf Remark.} Using the notation $\BCN (\Grad \cdot \BGX)$ for the Newton's potential acting on $\Grad \cdot \BGX$ we can interpret the integral in \eq{alg5m} as
$$
\Big(  \BCN (\Grad \cdot \BGX), \Grad \cdot \BGX  \Big)_{L_2({\Bbb R}^3)},
$$
since obviously $\Grad \cdot \BGX \in W^{-1,2}({\Bbb R}^3)$ and $\BCN (\Grad \cdot \BGX) \in W^{1,2}({\Bbb R}^3)$.  Here and in the sequel %of the paper 
we use the notation
$(  \Gvf, \psi )$ for the extension of the integral $\int_{{\Bbb R}^3} \Gvf (\BX) \psi(\BX) d \BX$ onto the Cartesian product $W^{1,2}({\Bbb R}^3) \times W^{-1,2}({\Bbb R}^3).$




{\bf Proof of Lemma \ref{lem1_alg}.}  %Consider the scalar product of \eq{alg1} and the vector $\BCP \BC$:
%\beq
%-\langle \BC, \BP \BC \rangle + \Gve^3 \langle \BCS \BP \BC, \BP \BC \rangle = \langle \BGT_f, \BP \BC \rangle.
%\eequ{alg6}
%The modulus of the right-hand side of \eq{alg6} does not exceed
%$$
%\langle  \BC, -\BP \BC \rangle^{1/2}  \langle \BGT_f, -\BP \BGT_f \rangle^{1/2}.
%$$
%The second term in the left-hand side of \eq{alg6}  can be expanded as
%The 
a) By \eq{alg2}, \eq{alg3}, the following representation holds
\beq
 \langle \BCS \BQ \BC, \BQ \BC \rangle 
 %\eequ{alg6a}
 %$$
 = \fr{1}{4 \pi} \sum_{j=1}^N   \Big(   \BCQ^{(j)} \BC^{(j)} \Big)^T  \sum_{1 \leq k \leq N, k \neq j} 
  (\nabla_{\Bz} \otimes \nabla_{\Bw})\left(\frac{1}{ |\Bz-\Bw|}\right)\Big|_{\substack{\Bz=\BO^{(j)}\\ \Bw=\BO^{(k)}}}  \Big(   \BCQ^{(k)} \BC^{(k)} \Big) .
 \eequ{alg6a}
%$$
Using the mean value theorem for harmonic functions we note that when $j \neq k$
$$
(\nabla_{\Bz} \otimes \nabla_{\Bw})\left(\frac{1}{ |\Bz-\Bw|}\right)\Big|_{\substack{\Bz=\BO^{(j)}\\ \Bw=\BO^{(k)}}} = \fr{3}{4 \pi (d/4)^3} \int_{B_{d/4}^{(k)}} 
(\nabla_{\Bz} \otimes \nabla_{\Bw})\left(\frac{1}{ |\Bz-\Bw|}\right)\Big|_{\substack{\Bz=\BO^{(j)}}} d \Bw.
$$
Substituting this identity into \eq{alg6a} and using %the 
 definition \eq{alg3a} we see that the inner sum on the right-hand side of \eq{alg6a} can be presented in the form
\begin{eqnarray}
%\langle  \BCS \BP \BC, \BP \BC  \rangle && = \fr{3}{4 \pi (d/4)^3} \sum_{j=1}^N \Big(   \BP^{(j)} \BC^{(j)} \Big)^T
%\nonumber \\
&& %\cdot 
\fr{48}{\pi d^3}  \lim_{\tau \to 0+} \int_{{\Bbb R}^3 \setminus B^{(j)}_{(d/4) - \tau} } \Big\{    \fr{\prt}{\prt Y_q}  \Big(   \fr{Y_r - O_r^{(j)}}{|\BY - \BO^{(j)}|^3}\Big)\Big\}_{q,r=1}^3 % \Big)  
\BGX(\BY) d\BY,
\nonumber 
\end{eqnarray}
and further integration by parts gives
\begin{eqnarray}
\langle  \BCS \BQ \BC, \BQ \BC  \rangle &&= - \fr{12}{\pi^2 d^3} \sum_{j=1}^N \Big(   \BCQ^{(j)} \BC^{(j)} \Big)^T
\label{alg7} \\
&&
\cdot \lim_{\tau \to 0+} \Bigg\{  
\int_{{\Bbb R}^3 \setminus B^{(j)}_{(d/4) - \tau} } \Big\{    \fr{Y_r - O_r^{(j)}}{|\BY - \BO^{(j)}|^3}  \Grad \cdot  \BGX(\BY)\Big\}_{r=1}^3 d\BY
\nonumber \\
&&
+ \int_{|\BY - \BO^{(j)}| = (d/4) -\tau} \Bigg\{  \fr{(Y_r - O_r^{(j)})  (Y_q- O_q^{(j)})}{|\BY - \BO^{(j)}|^4}   \Bigg\}_{r, q = 1}^3 d S_\BY ~\BCQ^{(j)} \BC^{(j)} \Bigg\}, \nonumber
\end{eqnarray}
where the integral over ${\Bbb R}^3 \setminus B_{(d/4) - \tau}$ in \eq{alg7} is understood in the sense of distributions. The surface integral  in \eq{alg7} can be evaluated explicitly, i.e.
\beq
\int_{|\BY - \BO^{(j)}| = (d/4) -\tau} \Bigg\{  \fr{(Y_r - O_r^{(j)})  (Y_q- O_q^{(j)})}{|\BY - \BO^{(j)}|^4}   \Bigg\}_{r, q = 1}^3 d S_\BY ~\BCQ^{(j)} \BC^{(j)} = \fr{4 \pi}{3} \BCQ^{(j)} \BC^{(j)}.
\eequ{alg8}
Once again, applying the mean value theorem for harmonic functions in the outer sum of  \eq{alg7} and using \eq{alg8} together with the definition \eq{alg3a} we arrive at
\begin{eqnarray}
\langle  \BCS \BQ \BC, \BQ \BC  \rangle &&= - \fr{16}{\pi d^3} \sum_{j=1}^N |   \BCQ^{(j)} \BC^{(j)} |^2
\label{alg9} \\
- \fr{576 %768
}{\pi^3 %2 
d^6 } && \lim_{\tau \to 0+}  
\sum_{j=1}^N \int_{ %{\Bbb R}^3 
B^{(j)}_{(d/4) + \tau}} \int_{{\Bbb R}^3 \setminus B^{(j)}_{(d/4) - \tau} }\sum_{r=1}^3 \GX_r(\BX) \fr{\prt}{\prt X_r}  \Big(\fr{1}{|\BY - \BX|}\Big)  \Grad \cdot  \BGX(\BY) d\BY d \BX,
\nonumber 
\end{eqnarray}
where $\Xi_r$ are the components of the vector function $\BGX$ defined in (\ref{alg3a}).
 
The last integral is understood in the sense of distributions. 
%Taking into account that the components of the vector function $\BGX$ are constant in $\ov{B}^{(j)}_{(d/4)-\tau}$ 
Referring to the definition  \eq{alg3a}, integrating by parts, and taking the limit as
$\tau \to 0+$ we deduce that
the integral term in \eq{alg9} can be written as 
\begin{eqnarray}
%- \fr{768}{\pi^2 d^6 } && 
%\int_{{\Bbb R}^3 } \int_{{\Bbb R}^3 }\sum_{r=1}^3 \GX_r(\BX) \fr{\prt}{\prt X_r}  \Big(\fr{1}{|\BY - \BX|}\Big)  \Grad \cdot  \BGX(\BY) d\BY d \BX \\
%= 
\fr{576 %768
}{\pi^3%2 
d^6 } && 
\int_{{\Bbb R}^3 } \int_{{\Bbb R}^3 }  \fr{1}{|\BY - \BX|} \Big( \Grad \cdot \BGX(\BX) \Big)  \Big( \Grad \cdot  \BGX(\BY) \Big) d\BY d \BX \label{alg10}
\end{eqnarray}
Using \eq{alg9} and \eq{alg10} we arrive at \eq{alg5m}. 

\vspace{.2in}

%It now follows from Lemma \ref{lem1_alg}, that 
%\begin{equation}\label{eqidentQC}
%\langle \BCS \BQ \BC, \BQ\BC\rangle=\frac{32}{\pi d^3}\langle \BQ\BC, \BQ\BC\rangle\;.
%\end{equation}
%To see this, one needs to only apply integration by parts twice to the integral term in (\ref{alg5m}). Upon the first application to the inner integral in (\ref{alg5m}) we obtain
%\begin{eqnarray*}
%\langle   \BCS \BQ \BC, \BQ \BC  \rangle &&= \fr{ 2304 %768
%}{\pi^2 %2 
%d^6}   \int_{\mathbb{R}^3} \nabla_{\BY}\cdot \BGX(\BY) \int_{\mathbb{R}^3} \nabla_{\BY} \Big(\frac{1}{4\pi|\BX-\BY|}\Big)\cdot \BGX(\BX)\, d\BX\, d\BY \nonumber \\
%&& - \fr{16}{ \pi d^3}
%\sum_{j=1}^N   | \BCQ^{(j)}  \BC^{(j)} |^2.
%\label{alg5ma}
%\end{eqnarray*}
%Then, repeating the procedure now to the outer  and using the definition (\ref{alg3a})  gives
%\begin{eqnarray*}
%\langle   \BCS \BQ \BC, \BQ \BC  \rangle &&= \fr{ 2304 %768
%}{\pi^2 %2 
%d^6}   \int_{\mathbb{R}^3}  \BGX(\BY)\cdot \int_{\mathbb{R}^3} \nabla_{\BY} \Big(\nabla_{\BY} \Big(\frac{1}{4\pi|\BX-\BY|}\Big)\cdot \BGX(\BX)\Big)\, d\BX\, d\BY \nonumber \\
%&& - \fr{16}{ \pi d^3}
%\sum_{j=1}^N   | \BCQ^{(j)}  \BC^{(j)} |^2\\
%&&=\fr{ 2304 %768
%}{\pi^2 %2 
%d^6} \sum_{j=1}^N \int_{B^{(j)}_{d/4}}|\BGX(\BY)|^2\,d\BY- \fr{16}{ \pi d^3}
%\sum_{j=1}^N   | \BCQ^{(j)}  \BC^{(j)} |^2\\
%&&=\frac{32}{\pi d^3}\langle \BQ\BC, \BQ\BC\rangle\;.
%\label{alg5mb}
%\end{eqnarray*}
b) Let us introduce a piece-wise constant function 
\[\BCC(\Bx)=\left\{\begin{array}{ll}
\BC^{(j)}\;, & \quad \text{when } \Bx \in \overline{B^{(j)}_{d/4}}\;, \quad j=1, \dots, N\;,\\
0\;,&\quad \text{otherwise}\;.
\end{array}\right.
\]
According to the system (\ref{R3formalgeq9}), $\nabla \times \BCC(\Bx)=\BO$, and one can use the representation
\begin{equation}\label{CeqgrW}
\BCC(\Bx)=\nabla W(\Bx)
\end{equation}
where $W$ is a scalar function with compact support, and (\ref{CeqgrW}) is understood in the sense of distributions. We give a proof for the case when all voids are spherical, of diameter $\varepsilon$, and hence $\BCQ^{(j)}=-\frac{\pi}{4}\varepsilon^3 I_3$, where $I_3$ is the identity matrix. Then according to (\ref{alg9}) we have 
\begin{eqnarray*}
|\langle  \BCS \BQ \BC, \BQ \BC\rangle| &\le& \frac{16}{\pi d^3} \sum_{1\le j\le N} |\BQ^{(j)} \BC^{(j)}|^2+\frac{36\varepsilon^6}{\pi d^3}\Big| \int_{\mathbb{R}^3}\int_{\mathbb{R}^3} \Big(\nabla_{\BX} W(\BX) \cdot \nabla_{\BX}\Big(\frac{1}{|\BY-\BX|}\Big)\Big)\Delta_{\BY} W(\BY)\, d\BY d\BX \Big| \\
&\le&\frac{16}{\pi d^3} \sum_{1\le j\le N} |\BQ^{(j)} \BC^{(j)}|^2+\frac{144\varepsilon^6}{d^3} \sum_{1 \le j\le N} \int_{B^{(j)}_{d/4}} |\nabla W(\BY)|^2\, d\BY\\
&\le &\frac{\text{const}}{ d^3} \sum_{1 \le j \le N}|\BCQ^{(j)} \BC^{(j)}|^2\;.
\end{eqnarray*}\hfill$\Box$

{\bf Proof of Theorem \ref{thm1_alg}.}  Consider the equation \eq{alg6}. The %modulus 
absolute value of its right-hand side  does not exceed
$$
\langle  \BC, -\BQ \BC \rangle^{1/2}  \langle \BGT,%_f, 
-\BQ \BGT%_f
 \rangle^{1/2}.
$$
Using Lemma 1 and part b) of Lemma 2 we derive
\begin{eqnarray}
\langle \BC, -\BQ \BC \rangle - \text{const} d^{-3}  \langle -\BQ \BC, -\BQ \BC \rangle \leq \langle  \BC, -\BQ \BC \rangle^{1/2}  \langle \BGT,%_f, 
-\BQ \BGT%_f 
\rangle^{1/2}, \nonumber
\end{eqnarray}
%which leads 
leading to
\begin{eqnarray}
\Big(1 -  \fr{\text{const}  %\Gve^3
}{ d^3}  \fr{\langle -\BQ \BC, -\BQ \BC \rangle}{\langle \BC, -\BQ \BC \rangle}  \Big) \langle \BC, -\BQ \BC \rangle^{1/2}  \leq  \langle \BGT,%_f, 
-\BQ \BGT%_f 
\rangle^{1/2},
\nonumber
\end{eqnarray}
%The latter 
which implies
\begin{eqnarray}
\Big(1 -  \text{const} %\Gve^3
  \frac{\Gl_{max}}{d^{3}} \Big)^2 \langle \BC, -\BQ \BC \rangle  \leq  \langle \BGT,%_f, 
-\BQ \BGT%_f 
\rangle .
\label{alg11}
\end{eqnarray}
%where $\Gl_{max}$ is the largest eigenvalue of the positive definite matrix $-\BQ$, which characterizes the shapes of the small %voids. 
The proof is complete. $\Box$ 

Assuming that the eigenvalues of the matrices $-\BCQ^{(j)}$
%characterizing the shapes of individual scaled voids $\Go^{(j)}$,  
are strictly positive %definite 
and satisfy the inequality \eq{Gl_min}, we also find that Theorem \ref{thm1_alg} %also 
%leads to the estimate:
yields 

%{\bf Corollary 1.} 
\begin{coro} \label{coro1_alg} 
%{\em 
Assume that %$\Gve
% \Gl_{max} < ~d^3 $, and 
the inequalities {\rm \eq{Gl_min}} hold for $\Gl_{max}$ and $\Gl_{min}$.
% the maximal and minimal eigenvalues of the matrix $-\BQ$.  
 Then the vector coefficients $\BC^{(j)}$ in the system {\rm \eq{alg1}} satisfy the estimate %inequality
\beq
\sum_{1 \leq j \leq N} |\BC^{(j)}|^2 \leq \mbox{\rm const  } d^{-3} \| \Grad v%_f
\|^2_{L^2(\Go)},  %(1- \fr{16 \Gve^3}{\pi d^3} \Gl_{max} )^{-2} \fr{\Gl_{max}}{\Gl_{min}} \sum_{1 \leq j \leq N} |\Grad v_f(\BO^{(j)})|^2
\eequ{alg12}
where the constant %depends on the shape of the %scaled 
%does not depend on the size of the voids $F^{(j)}, j=1,\ldots, N.$ %}
depends only on the coefficients $A_1$ and $A_2$ in {\rm \eq{Gl_min}}.
%$\Gl_{min}$ and $\Gl_{max}$ are the minimum and maximum eigenvalues of the positive definite matrix $-\BP$.}
\end{coro}

\begin{proof}
According to the inequality \eq{alg4} of Theorem \ref{thm1_alg} we deduce
\beq
\Gl_{min} \sum_{1 \leq j \leq N} |\BC^{(j)}|^2 \leq (1- \fr{\text{const} %\Gve^3
}{ d^3} \Gl_{max} )^{-2} \Gl_{max} \sum_{1 \leq j \leq N} |\Grad v%_f
(\BO^{(j)})|^2.
\eequ{alg12aa}
%where  $\Gl_{min}$ and $\Gl_{max}$ are the minimum and maximum eigenvalues of the positive definite matrix $-\BP$, and and they satisfy \eq{Gl_min} . %$\Gl_{min} >0$. 
We note  that $v$ %_f$ 
is harmonic in a neighbourhood of $\ov{\Go}$. Applying the mean value theorem
for harmonic functions together with the Cauchy inequality we write
$$
|\Grad v%_f
(\BO^{(j)})|^2 \leq \fr{48}{ \pi d^{3}} \|\Grad v%_f
\|^2_{L_2(B^{(j)}_{d/4})}.
$$ 
Hence, it 
%then 
follows from \eq{alg12aa} that
\begin{eqnarray}
 \sum_{1 \leq j \leq N} |\BC^{(j)}|^2 && \leq d^{-3} (1- \fr{\text{const} %\Gve^3
 }{ d^3} \Gl_{max} )^{-2}  \fr{48}{ \pi}  \fr{\Gl_{max}}{\Gl_{min}}    \sum_{1 \leq j \leq N} \|\Grad v%_f
 \|^2_{L_2(B^{(j)}_{d/4})} \nonumber \\
 && \leq d^{-3 }\left((1- \fr{\text{const} %\Gve^3
 }{ d^3} \Gl_{max} )^{-2} \fr{48}{\pi} \fr{\Gl_{max}}{ \Gl_{min}}  \right) \|\Grad v%_f
 \|^2_{L_2(\Go)},
\label{alg12b}
\end{eqnarray}
which %leads to 
is the required estimate \eq{alg12}.
\end{proof}

%\end{document}

==> Mesoscale pdf/boundformalg.tex <==
\section{%The a
Approximation of $u_N$ for %the case of 
a perforated %bounded 
domain}\label{boundformalg}
Now we seek %the 
an approximation of %$u_N$ 
the solution $u_N$  to the problem %(\ref{Mainnot1})--(\ref{Mainnot3}) 
\eq{intro_2}--\eq{intro_4} %for the situation when 
assuming that $\Omega$ is %a bounded 
an arbitrary domain in $\mathbb{R}^3$. We first describe the formal asymptotic algorithm and 
%show that the same
%derive another 
derive %the 
a system of algebraic equations, similar to \eq{alg1}, % Section \ref{R3alg}, 
 which is used %here 
 for evaluation of the coefficients in the asymptotic representation of $u_N$.
 
%as in Section whose solution plays a similar role to that of $\boldsymbol{C}^{(j)}$, $j=1, \dots, N$ in the previous sections.
%We now give the main result once more, then in the sequel we implement the formal asymptotic procedure


%Prior to the proof of the Theorem we describe the formal algorithm.
\subsection{Formal asymptotic algorithm for the %bounded 
perforated domain $\GO_N$}

The solution $u_N \in L^{1,2}(\GO_N)$  of  \eq{intro_2}--\eq{intro_4}   %(\ref{Mainnot1})--(\ref{Mainnot3}) 
is sought in the form 
\beq
u_N(\X)=v%_f
(\X)+ \sum_{k=1}^N \boldsymbol{C}^{(k)}\cdot \Big\{\BCD^{(k)}(\Bx) - %+ %\XI_k)+%\varepsilon^2 
\BCQ^{(k)}\nabla_\Y H(\X, \Y)\big|_{\Y=\Oj^{(k)}} \Big\}+R_N(\X)\;,
%R^{(1)}_N(\X)
%\;,
\eequ{u_N_0}
where in this instance $v$ %_f$ 
solves 
%Problem 1 
problem \eq{vfom_1}, \eq{vfom_2}   in  Section \ref{Modelproblems}, and $R%^{(1)}
_N$  is a harmonic function in $\Omega_N$.
% and has zero displacement on the exterior boundary. 
%On the % interior 
%boundaries of small voids $\partial F%\omega_\varepsilon
%^{(j)}$, $j=1, \dots, N$, the normal derivative of $R_N^{(1)}$ satisfies
%\begin{eqnarray}%\nonumber
%\label{boundformalgeq1}
%\Dn{R_N^{(1)}}{}(\X)&=&- \Dn{v_f}{}(\X)=-\N^{(j)}\cdot \nabla v_f(\X)  %\\
%%&=& 
%%=
%\sim -\N^{(j)} \cdot \nabla v_f(\Oj^{(j)})  %+O(\varepsilon)
%\;.
%\end{eqnarray}
%%where in the last equality we expanded the first order derivatives of $v_f$ about the centre $\Oj^{(j)}$ of the small void $%\omega_\varepsilon^{(j)}$.
%
%Next, we represent $R^{(1)}_N(\X)$ as 
%\begin{equation}\label{boundformalalgeq2}
%R_N^{(1)}(\X)=%\varepsilon 
%\sum_{k=1}^N \boldsymbol{C}^{(k)}\cdot \Big\{\BCD^{(k)}(\Bx) - %+ %\XI_k)+%\varepsilon^2 
%\BCQ^{(k)}\nabla_\Y H(\X, \Y)\big|_{\Y=\Oj^{(k)}} \Big\}+R_N(\X)\;,
%\end{equation}
%where 
Here $\boldsymbol{C}^{(k)}$, $k=1, \dots, N$ are the vector coefficients to be determined.
% later as a solution of certain  algebraic system. 

%Here. harmonicity of $R_N$ in $\Omega$ is guaranteed by the definitions of $R^{(1)}_N$, $\cD^{(k)}$, $k=1, \dots, N$ and $H$ (see Problems 2 and 3 of Section \ref{Modelproblems}). 
Owing to the definitions of $\BCD^{(k)}$, $k=1, \dots, N,$ and $H$ as solutions of Problems 2 and 3 in Section \ref{Modelproblems}, 
%the function $R_N$ is harmonic in $\GO_N$.
%On the exterior boundary, using 
and taking into account Lemma \ref{Djasymp} %including 
on the asymptotics of $\BCD^{(k)}$ %in (\ref{modfieldeq2}) %and the boundary condition for $H$,
 we deduce that $|R_N(\Bx)|$ is small for $\Bx \in \prt \GO.$
 %obtain 
%\beq |R_N(\X)|\leq \mbox{const } \varepsilon^4 \sum^N_{k=1}  |\boldsymbol{C}^{(k)}||\X-\Oj^{(k)}|^{-3} \;, \X \in \partial \Omega\;.\eequ{bdd_1a}
%Since the coefficients $\BC^{(k)}$ satisfy \eq{alg12}, and for all $\Bx \in \prt \GO$ and $\BO^{(k)}, k = 1,\ldots, N,$ we have $|\Bx - \BO^{(k)}| > h > 0$, then  the estimate \eq{bdd_1a} leads to
%\beq
%|R_N(\Bx)| \leq \mbox{const  } \Gve^4 \Big(  \sum_{k=1}^N   |\BC^{(k)}|^2 \Big)^{1/2} \Big(  \sum_{k=1}^N  |\Bx- \BO^{(k)}|^{-6} %\Big)^{1/2} \leq \mbox{const  }  \Gve^4 d^{-3} \|\Grad v_f \|_{L_2}(\Go), ~~ \Bx \in \prt \GO.
%\eequ{bdd_11}


On the boundaries %of small voids 
$\prt F% \Go_\Gve
^{(j)}$, the substitution of (\ref{u_N_0}) %boundformalalgeq2}) 
into (\ref{intro_4}) %boundformalgeq1}) 
yields
\begin{eqnarray*}
\Dn{{R}_N}{}(\X)&=&-\N^{(j)} \cdot \Big\{ \nabla v%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)}+O(\varepsilon)+O(\varepsilon^3 |\boldsymbol{C}^{(j)}|)
\\&&+ %\varepsilon 
\sum_{\substack{k \ne j\\ 1 \le k \le N}} \nabla \Big\{ \boldsymbol{C}^{(k)} \cdot \Big(\BCD^{(k)}(\Bx %XI_k
)  - %+ %\varepsilon^2 
\BCQ^{(k)}\nabla_\Y H(\X, \Y)\big|_{\Y=\Oj^{(k)}} \Big) \Big\}\Big\}
%+ O\left(\varepsilon^3 \sum^N_{k=1} |\boldsymbol{C}^{(k)}|\right)\Big\} 
\;, \quad \X \in  \partial F%\omega_\varepsilon
^{(j)}, j=1, \dots, N\;.
\end{eqnarray*}
Then, using the asymptotic representation (\ref{modfieldeq2}) %from 
in Lemma \ref{Djasymp} we deduce
\begin{eqnarray} %\nonumber 
\label{boundformalalgeq3}
\Dn{{R}_N}{}(\X)&\sim&-\N^{(j)}\cdot\Big\{ \nabla v%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)}%+O(\varepsilon) 
+    %\varepsilon^3 
\sum_{\substack{k \ne j \\ 1 \le k \le N}} {\frak T}(\X, \Oj^{(k)})\BCQ^{(k)} \boldsymbol{C}^{(k)}  %\\
%&&+O\Big(\sum_{\substack{k \ne j \\ 1 \le k \le N}} \frac{\varepsilon^4 |\boldsymbol{C}^{(k)}|}{|\X -\Oj^{(k)}|^4}\Big) %+ O\Big(\varepsilon^3 \sum^N_{k=1} |\boldsymbol{C}^{(k)}|\Big)
\Big\}\;, \quad \X \in \partial F %\omega_\varepsilon
^{(j)}, j=1, \dots, N\;,
\end{eqnarray}
where ${\frak T(\X, \Y)}$ is defined by %
\begin{equation}\label{defFT}
{\frak T}(\X, \Y)=(\nabla_{\X} \otimes \nabla_{\Y}) G(\X, \Y)  \;,
\end{equation} %the same as in \eq{defT}.
with $G(\X, \Y)$ being Green's function for the 
%limit 
domain $\GO$, as defined in Section \ref{Modelproblems}.
%\[T(\X, \Y)=(\nabla_{\bZ} \otimes \nabla_{\bW})\left( \frac{1}{4\pi|\bZ-\bW|}\right)\Big|_{\substack{\bZ=\X\\ \bW=\Y}}\;.\]
%When $j \neq k$, %The Taylor expansion of $T(\X, \Oj^{(k)})$ about $\X =\Oj^{(j)}$ in
%\eq{boundformalalgeq3} and (\ref{boundformalalgeq3}) lead to
%\begin{eqnarray}   \label{bdd_2}
%\Dn{\mathcal{R}_N}{}(\X)&\sim&-\N^{(j)}\cdot\Big\{ \nabla v_f(\Oj^{(j)})+\boldsymbol{C}^{(j)}  %+O(\varepsilon) 
%-  %\varepsilon^3 
%\sum_{\substack{k \ne j \\ 1 \le k \le N}} {\frak T}(\Oj^{(j)}, \Oj^{(k)})\BCQ^{(k)} \boldsymbol{C}^{(k)}   % \nonumber \\
%%&&+O\Big(\sum_{\substack{k \ne j \\ 1 \le k \le N}} \frac{\varepsilon^4 |\boldsymbol{C}^{(k)}|}{|\X -\Oj^{(k)}|^4}\Big) %+ O%\Big(\varepsilon^3 \sum^N_{k=1} |\boldsymbol{C}^{(k)}|\Big)
%\Big\}\;, \quad \X \in \partial F%\omega_\varepsilon
%^{(j)}, j=1, \dots, N\;. \label{bdd_2}
%\end{eqnarray}
To compensate for the leading discrepancy %, produced by the terms $\nabla v_f(\Oj^{(j)})+\boldsymbol{C}^{(j)} -\varepsilon^3 \sum_{\substack{k \ne j \\ 1 \le k \le N}} T(\Oj^{(j)}, \Oj^{(k)})\cP^{(k)} \boldsymbol{C}^{(k)}$  
in the boundary conditions \eq{boundformalalgeq3}, %bdd_2},
we choose  the coefficients $\boldsymbol{C}^{(m)}$, $m=1, \dots, N,$ 
%in such a way that they  satisfy
subject to  the algebraic system %(\ref{R3formalgeq9}).
\beq
\nabla v
%_f
(\Oj^{(j)})+\boldsymbol{C}^{(j)} +%\varepsilon^3 
\sum_{\substack{k \ne j \\ 1 \le k \le N}} {\frak T}(\Oj^{(j)}, \Oj^{(k)})
%\cP^{(k)}
\BCQ%_\Gve
^{(k)} \boldsymbol{C}^{(k)}=0, ~~ j =1, \ldots,N,
\eequ{R3formalgeq9a}
%In order to prove Theorem \ref{mainthm1}, in the next section we give the energy estimate for $R_N$.
%In the next section we formulate Theorem \ref{mainthm1} on the asymptotic approximation of $u_n$ and will provide the remainder estimate.
where $\BCQ%_\Gve
^{(k)}, k=1,\ldots,N,$ are polarization matrices of small voids $%\Go_\Gve
F^{(k)}$, as  in Lemma \ref{Djasymp}. %\eq{P_eps}.

Provided %the 
system \eq{R3formalgeq9a} has been solved for the vector coefficients $\BC^{(k)}$, %the 
 formula \eq{u_N_0} %, %\eq{boundformalalgeq2} 
leads to the formal asymptotic approximation of $u_N$:
\beq
u_N(\Bx) \sim v%_f
(\Bx) + \sum_{k=1}^N \boldsymbol{C}^{(k)}\cdot \Big\{\BCD^{(k)}(\Bx) - %+ %\XI_k)+%\varepsilon^2 
\BCQ^{(k)}\nabla_\Y H(\X, \Y)\big|_{\Y=\Oj^{(k)}} \Big\}.
\eequ{u_N_formal}


\subsection{Algebraic system} % for the case of a bounded domain}

The system \eq{R3formalgeq9a} can be written in  the matrix form
 \beq
\BC + %\Gve^3 
{\frak S} \BQ \BC = - \BGT, %_f,
\eequ{alg11a}
where
\beq
{\frak S}=[{\frak S}_{ij}]_{i, j=1}^N, ~ 
{\frak S}_{ij}=\left\{\begin{array}{ll}\displaystyle{(\nabla_{\Bz} \otimes \nabla_{\Bw})G(\Bz, \Bw )\Big|_{\substack{\Bz=\BO^{(i)}\\ \Bw=\BO^{(j)}}}} & \quad \text{ if } i \ne j\\
& \\
{0}I_3 %\BI_3
&\quad \text{otherwise}\end{array}  \right.  
\eequ{alg22a}
with $G(\Bz, \Bw)$ %being 
standing for Green's function in the limit domain $\GO$,
and the block-diagonal matrix $\BQ$ being the same as in \eq{matrix_Q}. % and accordingly the vector representation \eq{alg1} of the system becomes
% The system   \eq{R3formalgeq9a} 
%It
The system \eq{alg11a} is similar to that % he system  studied 
in Section \ref{alg_syst}, with the only change %being  
%in the replacement 
of the matrix $\BCS$ %$T(\Oj^{(j)}, \Oj^{(k)})$ 
%by 
for ${\frak S}$. %${\frak T}(\Oj^{(j)}, \Oj^{(k)})$.
%whose components
The elements of  ${\frak S}$ are given via the second-order derivatives of Green's function in $\GO$, as defined in \eq{defFT}. 
%As before, we consider the case when the matrices $-\BCQ^{(j)}$ from \eq{u_N_formal}
%, characterizing the shapes of
%individual scaled voids $\Go^{(j)}$ 
%are strictly positive definite, and their maximal and minimal eigenvalues satisfy \eq{Gl_min}.  
%we give the statement on solvability of \eq{R3formalgeq9a}
The next assertion is similar to Corollary \ref{coro1_alg}.

%\begin{thm} 
 \begin{lem}  \label{thm1_alg_f} 
%{\em 
%Assume that $\Gve < c~d $, where $c$ is a sufficiently small absolute constant, and 
%==
Assume that 
%the 
inequalities {\rm \eq{Gl_min}} hold for $\Gl_{max}$ and $\Gl_{min}$. 
%, the maximal and minimal eigenvalues of the matrix 
%$-\BQ$. 
Also 
let $v%_f
$ be a unique solution of %the model 
problem {\rm \eq{vfom_1}, \eq{vfom_2}} in the
%limit 
domain $\GO$.  
%Also assume that for the positive definite matrices $-\BCQ^{(k)}$ in {\rm \eq{R3formalgeq9a}}, their minimal and maximal %eigenvalues satisfy 
%{\rm \eq{Gl_min}}.  Then the algebraic system 
%{\rm \eq{R3formalgeq9a}} is solvable and 
Then the vector coefficients $\BC^{(j)}$ in the system {\rm \eq{R3formalgeq9a}} satisfy the estimate % }
%==
\beq
\sum_{1 \leq j \leq N} |\BC^{(j)}|^2 \leq \mbox{\rm const} ~ d^{-3} \| \Grad v%_f
 \|^2_{L^2(\GO)}, 
%====  \sum_{1 \leq j \leq N} |\Grad v_f(\BO^{(j)})|^2.
\eequ{alg12a}
%===
where the constant depends on the shape of the voids $F^{(j)}, j= 1,\ldots, N.$
%\end{thm}
\end{lem}

\begin{proof}
The proof of the theorem is very similar to the one given in Section \ref{alg_syst}. We consider the scalar product of \eq{alg11a} and the vector $\BQ \BC$:
\beq
\langle \BC, \BQ \BC \rangle + \langle {\frak S} \BQ \BC, \BQ \BC \rangle =  -\langle  \BGT%_f
, \BQ \BC \rangle,
\eequ{alg112a}
and similarly to \eq{alg5m} derive


%Although the proof of the theorem is very similar to the one given in Section \ref{alg_syst}, there are some differences due to the contribution from the exterior boundary $\prt \GO$, which will be outlined here.
%First, the matrix  $\BCS$ in \eq{alg2} is replaced by a $3N \times 3N$ matrix ${\frak S}$ defined in \eq{alg22a}, where
%\beq
%{\frak S} = \BCS - {\frak H},
%\eequ{frakS_vs_H}
%and the matrix components of %the %matrix 
%${\frak H}$ are 
%\beq
%{\frak H}_{ij}=\left\{\begin{array}{ll}\displaystyle{(\nabla_{\Bz} \otimes \nabla_{\Bw})\left(H(\Bz, \Bw)\right)\Big|_{\substack{\Bz=\BO^{(i)}\\ \Bw=\BO^{(j)}}}}, & \quad \text{ if } i \ne j,\\
%& \\
%{\bf 0}, %\BI_3
%&\quad \text{otherwise},\end{array}  \right.  
%\eequ{frakH}
%with $H$ being the regular part of Green's function in $\GO$.
%
%Then it follows from \eq{alg5m} and \eq{frakS_vs_H} that 
%\begin{eqnarray}
%\langle   {\frak S} \BQ \BC, \BQ \BC  \rangle &&= 576~ \pi^{-3%2
%}~ d^{-6} \int_{\GO}  \int_{\GO} %G( \BX, \BY) 
%|\BX-\BY|^{-1} (\Grad \cdot \BGX(\BX))  (\Grad \cdot \BGX(\BY)) d \BY  d \BX \nonumber \\
%&& - 16 \pi^{-1} d^{-3}
%\sum_{j=1}^N   | \BCQ^{(j)}  \BC^{(j)} |^2 - \langle   {\frak H} \BQ \BC, \BQ \BC  \rangle, \label{frSH}
%\end{eqnarray}
%Let us consider the last term in \eq{frSH}:
%\begin{eqnarray}
%\langle   {\frak H} \BQ \BC, \BQ \BC  \rangle  && =\sum_{1 \leq j \leq N}   \Big(   \BCQ^{(j)} \BC^{(j)} \Big)^T  \sum_{1 \leq k \leq N} 
%  (\nabla_{\Bz} \otimes \nabla_{\Bw})\left(H(\Bz, \Bw)\right)\Big|_{\substack{\Bz=\BO^{(j)}\\ \Bw=\BO^{(k)}}}  \Big(   \BCQ^{(k)} \BC^{(k)} \Big) \nonumber \\
 %&& -\sum_{1 \leq j \leq N}   \Big(   \BCQ^{(j)} \BC^{(j)} \Big)^T 
 % (\nabla_{\Bz} \otimes \nabla_{\Bw})\left(H(\Bz, \Bw)\right)\Big|_{\substack{\Bz=\BO^{(j)}\\ \Bw=\BO^{(j)}}}  \Big(   \BCQ^{(j)} %\BC^{(j)} \Big) .
%\label{frH1}
%\end{eqnarray}
%Using the notation $\BGX$, defined in \eq{alg3a}, together with the mean value theorem for harmonic functions we write the first sum in \eq{frH1} as
%\beq
%\fr{(48)^2}{\pi^2 d^6} \int_\GO \int_\GO \sum_{1 \leq r,q \leq 3} \BGX_r (\BX)  \BGX_q (\BY) \fr{\prt^2}{\prt X_r \prt Y_q}H(\BX, \BY) d\BX d \BY.  
%\eequ{frH2}
%Integrating \eq{frH2} twice by parts and substituting the result into \eq{frSH} we obtain
%%
%%Furthermore, with the notation $\BGX$ being the same as in \eq{alg3a} the identity \eq{alg5m} is replaced by
\begin{eqnarray}
\langle   {\frak S} \BQ \BC, \BQ \BC  \rangle &&= %3072
%576
48^2~ \pi^{-2%2
}~ d^{-6} \int_{\GO}  \int_{\GO} %G( \BX, \BY) 
%|\BX-\BY|^{-1} 
G(\BX, \BY)(\Grad \cdot \BGX(\BX))  (\Grad \cdot \BGX(\BY)) d \BY  d \BX \nonumber \\
&& - 16 \pi^{-1} d^{-3}
\sum_{1 \le j \le N }  | \BCQ^{(j)}  \BC^{(j)} |^2  \nonumber \\
&& + \sum_{1 \leq j \leq N}   \Big(   \BCQ^{(j)} \BC^{(j)} \Big)^T 
  (\nabla_{\Bz} \otimes \nabla_{\Bw})\left(H(\Bz, \Bw)\right)\Big|_{\substack{\Bz=\BO^{(j)}\\ \Bw=\BO^{(j)}}}  \Big(   \BCQ^{(j)} \BC^{(j)} \Big) ,
\label{alg5new}
\end{eqnarray}
where the integral in the right-hand side is positive, and it is understood in the sense of distributions, in the same way as in the proof of Lemma \ref{lem1_alg}, while the magnitude of the last sum in \eq{alg5new} is small compared to the magnitude of the second sum. 

Now, %consider the equation \eq{alg112a}. Its 
the right-hand side in \eq{alg112a} does not exceed
$$
\langle  \BC, -\BQ \BC \rangle^{1/2}  \langle \BGT, %_f,
 -\BQ \BGT%_f 
 \rangle^{1/2}.
$$
%Using the positivity of the integral on the right-hand side in \eq{alg5new} we deduce
Following the same pattern as in the proof of Theorem \ref{thm1_alg}, we deduce
\begin{eqnarray}
\langle \BC, -\BQ \BC \rangle - \mbox{const } d^{-3}  \langle -\BQ \BC, -\BQ \BC \rangle \leq \langle  \BC, -\BQ \BC \rangle^{1/2}  \langle \BGT%_f
, -\BQ \BGT%_f 
\rangle^{1/2}, \nonumber
\end{eqnarray}
where the constant is independent of $d$. Furthermore, this leads to 
\begin{eqnarray}
\Big(1 -  \mbox{const } d^{-3}  \fr{\langle -\BQ \BC, -\BQ \BC \rangle}{\langle \BC, -\BQ \BC \rangle}  \Big) \langle \BC, -\BQ \BC \rangle^{1/2}  \leq  \langle \BGT%_f
, -\BQ \BGT%_f
 \rangle^{1/2},
\nonumber
\end{eqnarray}
which implies
\begin{eqnarray}
\Big(1 -  \mbox{const } d^{-3} \Gl_{max} \Big)^2 \langle \BC, -\BQ \BC \rangle  \leq  \langle \BGT,%_f, 
-\BQ \BGT%_f 
\rangle,
\label{alg1111}
\end{eqnarray}
where $\Gl_{max}$ is the largest eigenvalue of the positive definite matrix $-\BQ$.
Then using the same estimates \eq{alg12aa} and  \eq{alg12b} as in the proof of  Corollary
\ref{coro1_alg} we arrive at \eq{alg12a}.
\end{proof}


\subsection{%The e
Energy estimate for the remainder}\label{boundenergyestRN}

\begin{thm}\label{mainthm1}
Let the parameters $\varepsilon$ and $d$ satisfy the inequality
\[\varepsilon < c\, d   %|\log d|^{-1/3}
\;,\]
where $c$ is a sufficiently small absolute constant. Then the solution $u_N(\X)$ of %{\rm (\ref{Mainnot1})--(\ref{Mainnot3})}  
{\rm \eq{intro_2}--\eq{intro_4}}   is represented by the asymptotic formula
\begin{equation}\label{introeq1a}
u_N(\X)=v(\X)+ %\varepsilon
 \sum^N_{k=1} \boldsymbol{C}^{(k)} \cdot \{ %\Gve
  \BCD^{(k)}(\Bx) %\XI_k)
 - %+ %\varepsilon^2 
 %\cP_\Gve
 \BCQ^{(k)} \nabla_\Y H(\X, \Y)\Big|_{\Y=\Oj^{(k)}}\}+R_N(\X)\;,
\end{equation}
where $\boldsymbol{C}^{(k)}=(C^{(k)}_1, C^{(k)}_2, C^{(k)}_3)^T$%, and  the column vector $\mathbf{C}=(C^{(1)}_1, C^{(1)}_2, C^{(1)}_3, \dots, C^{(N)}_1, C^{(N)}_2, C^{(N)}_3)^T$ is given by
solve the linear algebraic system {\rm \eq{R3formalgeq9a}}. %{\rm \eq{alg1}} with the matrix
%\beq%\mathbf{\Xi}_f=(
%\mathbf{I}-\varepsilon^3 \BCS\mathbf{P}%\mathbf{C}\;
%.\eequ{bdd_1}
%The matrix {\rm \eq{bdd_1}} %$(\mathbf{I}+\varepsilon^3 \mathbf{S}\mathbf{P})$ 
%is invertible and the 
The remainder $R_N$ in {\rm \eq{introeq1a}} satisfies the energy
estimate
\begin{equation}\label{introeq2a}
 \| \nabla R_N\|^2_{L_2(\Omega_N)} \le \text{\emph{const} } \Big\{ \varepsilon^{11}d^{-11}  + \varepsilon^{5}d^{-3}  \Big\}  \| \nabla v%_f
 \|^2_{L_2(\Omega)}
 %+
 %\,d^{2}       %\max_{1 \le i, j \le 3}\Big\| \frac{\partial^2 v_f}{\partial x_i \partial x_j} \Big\|^2_{L_\infty(\omega)}
 %\|v_f \|_{L_2 (\Go_h)}^2
% \Big\}
\;.
 \end{equation}
% where $\Go_h$ is the same as in Theorem {\rm \ref{R3thmasy}}.
\end{thm}

%{\bf Proof:}
%\begin{proof}
%In this section we direct our attention  to the energy estimate for the remainder $R_N$ present in the approximation (\ref{introeq2a}).

%\begin{lem}\label{boundenestproof}
%Let the small parameters $\varepsilon$ and $d$ defined, in Section $\ref{MainNotmeso}$ satisfy
%\[\varepsilon \le c \, d\;,\]
%where $c$ is a sufficiently small absolute constant. Then the remainder $R_N$ in (\ref{introeq1a}) satisfies the estimate
%\begin{equation}\label{boundenesteq1}
%\| \nabla R_N\|_{L_2 (\Omega_N)} \le \text{const } \Big\{\varepsilon^{4} d^{-7/2} \| \nabla v_f\|_{L_\infty(\omega)}+\varepsilon d^{-1} \max_{1 \le i , j \le N} \Big\|\frac{\partial^2 v_f}{\partial x_i \partial x_j}\Big\|_{L_\infty(\omega)}\Big\}\;.
%\end{equation} 
%\end{lem}
{\it Proof. } Essentially, the proof follows the same steps as in %the proof of 
Theorem %\ref{R3thmasy}
\ref{thm1_alg_f_inf}. Thus, we give an outline indicating the obvious modifications, which are brought 
%due to the contribution from the exterior 
by the boundary $\prt \GO.$ 


\emph{a) Auxiliary functions. } Let us preserve the notations $\chi_\Gve^{(k)}$ for cutoff functions used in the proof of Theorem \ref{thm1_alg_f_inf}. We also
need a new cutoff function $\chi_0$ to isolate $\prt \GO$ from the cloud of holes. Namely, let $(1-\chi_0) \in C_0^\infty(\GO)$
and $\chi_0 = 0$ on a neighbourhood of $\ov{\Go}$. A neighbourhood of $\prt \GO$ containing $\mbox{supp } \chi_0$ will be denoted by $\CV$.
%
%We need additional auxiliary functions to deal with the new features attributed to the presence of the exterior boundary $\partial \Omega$. 
%%Then we sketch the derivation of the analogue of (\ref{R3ineq}), followed by the proof Theorem \ref{mainthm1}.
%
%\emph{a) Auxiliary functions. }First, let $\CV_s$ %\Omega_d$ 
%be a $s$-neighbourhood of the exterior boundary $\partial \Omega$: ~~
%$\CV_s = \{\Bx: \mbox{dist}(\Bx, \prt \GO) < s \}$. A smooth cut-off function $\chi_0(t)$ is defined in such a way that $\chi_0(%d^{-1}
%\Bx) = 1$ for all $\Bx \in \CV_{h/2 %d/4
%}$, and
%$\chi_0(%d^{-1}
%\Bx) = 0$ for all $\Bx \in {\Bbb R}^3 \setminus \ov{\CV}_{h %d/2
%}$, where $h$ is the same as in the definition \eq{intro_1}. 
%Also we use the cut-off functions $\chi^{(k)}_\Gve %k\big((\Bx - \BO^{(k)})/\Gve \big)
%$ defined in part (b) of the proof of Theorem 
%\ref{thm1_alg_f_inf}.
%%\ref{R3thmasy}. 
Instead of the functions $\Psi_k$ defined in \eq{R3energyest3}, we introduce
\begin{eqnarray}\label{R3energyest3_bdd}\nonumber
\Psi^{(\GO)}_k(\X)&=&v%_f
(\X)-v
%_f
(\BO^{(k)})-(\X-\Oj^{(k)})\cdot \nabla v%_f
(\Oj^{(k)})+ %\varepsilon 
\sum_{\substack{j \ne k\\ 1 \le j \le N}} \boldsymbol{C}^{(j)} \cdot \BCD^{(j)}(  \Bx %\XI_j
)\\
&&-%\varepsilon^3 
\sum_{\substack{j \ne k \\ 1 \le j \le N}} (\X-\Oj^{(j)})\cdot {\frak T}(\Oj^{(k)}, \Oj^{(j)}) \BCQ^{(j)}\boldsymbol{C}^{(j)}-\sum_{j=1}^N \boldsymbol{C}^{(j)} \cdot \BCQ^{(j)} \nabla_\By H(\Bx, \By)\Big|_{\By=\BO^{(j)}}\;, 
\end{eqnarray}
where the matrix ${\frak T}$ is defined in \eq{defFT} via second-order derivatives of Green's function in $\GO$. Owing to \eq{introeq1a} and the algebraic system \eq{R3formalgeq9a} we have
\beq
\fr{\prt}{\prt n} \left( \Psi_k^{(\GO)}(\Bx) + R_N(\Bx)  \right) = 0, ~~ \Bx \in \prt F %\Go_\Gve
^{(k)}.
\eequ{bcond_psi}

We also
 use the  function
\begin{equation}\label{energyestbound1}
\Psi_0(\X)=  %\varepsilon 
\sum^N_{j=1} \boldsymbol{C}^{(j)}\cdot\big\{\cD^{(j)}(\Bx ) %\XI_j)
 - %\varepsilon^2 
 \BCQ^{(j)}\frac{(\X-\Oj^{(j)})}{4 \pi |\X-\Oj^{(j)}|^3}\big\}\;,
\end{equation}
which is harmonic in $\Omega_N$.  It follows from \eq{introeq1a} that 
%satisfies condition
\begin{equation}
R_N(\X)+\Psi_0(\X)=-\sum_{1 \leq j \leq N} \BC^{(j)} \cdot  \BCQ^{(j)} \Big\{ \frac{(\X-\Oj^{(j)})}{4 \pi |\X-\Oj^{(j)}|^3} -  \nabla_\Y H(\X, \BY)\Big|_{\BY=\BO^{(j)}} \Big\}  =0 \;, \quad \X \in \partial  \Omega\;. \label{psi0_bcond}
\end{equation}
% and we have an additional cut-off function defined by
%\[\Delta P_0(\X)=0\;, \quad \X \in \Omega_d \cap\Omega\;,\]
%\[ P_0(\X)=1\;,\quad \X \in \partial \Omega\;,\]
%\[ P_0(\X)=0\;, \quad \X \in \partial (\Omega_d \cap \Omega) \backslash \partial \Omega\;,\]
%and this function is extended by zero in $\Omega \backslash \Omega_d $ and the derivatives of $P_0$ satisfy the inequality
%\begin{equation}\label{boundenesteq2a}
%|\nabla P_0(\X)| =O(d^{-1})\;, \quad \text{ for } \X \in \Omega_d \cap \Omega\;.
%\end{equation}

\emph{b) The energy estimate for $R_N$. % versus $P_k$, $\Psi_k$, $k=0, \dots, N$.
} 
%In order to 
%%cope with the additional 
%take into account the 
%contribution brought
%by the exterior boundary, we employ  the function
We start with the identity
%\[R_N(\X)+%P_0(\X) 
%\chi_0(%d^{-1}
%\Bx)\Psi_0(\X). \]
%Using \eq{bcond_psi}, \eq{psi0_bcond} and integrating %this 
%by parts 
%%with $R_N (\Bx) + \sum_{1 \leq k \leq N} \chi_k(d^{-1} (\Bx-\BO^{(k)}))\Psi^{(\GO)}_k(\Bx)$, 
%we obtain the identity 
 \begin{eqnarray}
  && \int_{\GO_N}\nabla \Big({R}_N
  %(\X) 
  + \chi_0
  %(\Bx) %d^{-1} 
  \Psi_0
  %(\Bx) 
  \Big) \cdot \nabla \Big( {R}_N
  %(\X)  
   + \sum_{1 \leq k \leq N} \chi^{(k)}_\Gve %k\Big( %d^{-1} 
  %(\Bx - \BO^{(k)})/\Gve\Big) 
  \Psi^{(\GO)}_k
  %(\Bx) 
  \Big)\, d\X \nonumber \\
   &&
   = - \int_{\GO_N}\Big({R}_N %(\X) 
   + \chi_0 %( \Bx)%d^{-1} 
   \Psi_0 %(\Bx) 
    \Big)  \GD \Big( {R}_N %(\X)  
     + \sum_{1 \leq k \leq N} \chi^{(k)}_\Gve %k\Big( %d^{-1} 
   %(\Bx - \BO^{(k)}) / \Gve\Big) 
   \Psi^{(\GO)}_k %(\Bx) 
   \Big)\, d\X, % \nonumber  \\
   %&&~~~ + \int_{\prt B_R} \CR_N(\Bx) \fr{\prt}{\prt n} \CR_N(\Bx) d s_\X.
    \label{rem_1_bdd}
  \end{eqnarray}
  which follows from \eq{bcond_psi}, \eq{psi0_bcond}  by Green's formula. 
  According to the definitions of 
  %the cut-off functions 
  $\chi_0$ and $\chi^{(k)}_\Gve$, we have $\mbox{supp } \chi_0 %(\Bx) 
   \cap \mbox{supp } \chi^{(k)}_\Gve %k((\Bx-\BO^{(k)})/\Gve) 
   = \emptyset$ 
   for all $k=1,\ldots,N$.
  Hence the integrals in \eq{rem_1_bdd} involving the products of $\chi_0$ and $\chi^{(k)}_\Gve$ or their derivatives are equal to zero. Thus, using that $\GD R_N = 0 $ on $\GO_N$, we reduce % the equation 
  \eq{rem_1_bdd} 
% can be reduced  to
 to the equality 
  \begin{eqnarray}
 && \int_{\GO_N} |\Grad R_N %(\Bx)
 |^2 d \Bx + \sum_{1 \leq k \leq N} \int_{B_{3 \Gve} \setminus \ov{F %\Go}_\Gve
 }^{(k)}} \Grad R_N %(\Bx) 
 \cdot \Grad \Big(  \chi^{(k)}_\Gve %k(%\fr
 %({\Bx - \BO^{(k)}})/{\Gve}) 
 \Psi^{(\GO)}_k
 %(\Bx) 
 \Big) d\Bx +  \int_{\GO_N \cap \CV%_{h %d/2
  %}
  } \Grad R_N
  %(\Bx) 
  \cdot \Grad \Big(  \chi_0
  %(\Bx %\fr{\Bx - \BO^{(k)}}{d}
  %) 
  \Psi%^{(\GO)}
  _0
  %(\Bx) 
  \Big) d\Bx\label{rem_2_bdd}\\
  &&  = -  \sum_{1 \leq k \leq N} \int_{\GO_N} R_N
  %(\Bx) 
  \GD \left( \chi^{(k)}_\Gve %k(%\fr
%  ({\Bx - \BO^{(k)}})/{\Gve}) 
  \Psi^{(\GO)}_k
  %(\Bx) 
   \right) d\Bx, \nonumber
  \end{eqnarray}
 % We note that \eq{bcond_psi} and \eq{psi0_bcond} were used in the derivation of  \eq{rem_1_bdd} and \eq{rem_2_bdd} .
  which differs  in the left-hand side from \eq{rem_1BB} only by the integral over $\GO_N \cap \CV$.
  
  Similarly to the part (b) of the proof of Theorem \ref{thm1_alg_f_inf}  %\ref{R3thmasy} 
  we deduce
  \begin{eqnarray}
&& \| \Grad \CR_N \|^2_{L^2(\GO_N)} \leq \mbox{const}\Big\{  \|   \Grad \Psi_0 \|^2_{L^2(\GO \cap \CV%_{h%d/2
%}
)}  + %d^{-2} 
\|   \Psi_0 \|^2_{L^2(\GO \cap \CV%_{h%d/2
%}
)} 
%\nonumber \\
%&& 
+ \sum_{1 \leq k \leq N} %\Big( 
\|   \Grad \Psi_k \|^2_{L^2(B_{3 \Gve}^{(k)} % \setminus \ov{\Go}_\Gve^{(k)}
)} 
% + d^{-2} \|   \Psi_k \|^2_{L_2(B_{d/4}^{(k)} \setminus \ov{\Go}_\Gve^{(k)})}   
% \Big) 
\Big\}. \label{rem_3_bdd}
\end{eqnarray}


%Repeating %the 
Similar to the %all 
steps of part (d) of the proof %of 
in Theorem \ref{thm1_alg_f_inf},  %{R3thmasy}, 
%we %consider the second sum on the right-hand side of  \eq{rem_3_bdd} and 
%show that %it is 
%estimated 
the last sum is majorized by 
%the right-hand side in  \eq{introeq2a}. 
\beq
\mbox{const } (\Gve^{11} d^{-11} + \Gve^5 d^{-3} ) \| \Grad v%_f 
\|_{L^2(\GO)}^2.
\eequ{bound_new}
It remains to estimate 
%$\|   \Grad \Psi_0 \|^2_{L_2(\GO \cap \CV_{h %d/2
%})}  + %d^{-2} 
%\|   \Psi_0 \|^2_{L_2(\GO \cap \CV_{h %d/2
%})} $. 
two terms in \eq{rem_3_bdd} containing $\Psi_0$. Using \eq{R3energyest14}, %and \eq{R3energyest14a}, 
together with %the
%estimate 
\eq{alg12a}  we deduce 
\begin{eqnarray}
&&%d^{-2} 
\|\Psi_0
%(\Bx)
\|^2_{L^2 (\GO \cap \CV%_{h %d/2
%}
)} \leq \mbox{const} ~ %d^{-2} 
\Gve^8 \sum_{1 \leq j \leq N} \int_{\GO \cap \CV%_{h %d/2
%}
} \fr{|C^{(j)}|^2 d \Bx}{|\Bx - \BO^{(j)}|^6} \nonumber \\
&& \leq \mbox{const  } %\fr{
\Gve^8%}{d^3 %5
%} 
\sum_{1 \leq j \leq N} |C^{(j)}|^2 \leq \mbox{const} \fr{\Gve^8}{d^3 %6 %8
} \|\Grad v%_f
\|^2_{L^2(\GO)},  \label{rem_4_bdd_a}
\end{eqnarray}
%Similarly, for 
%For the remaining term %in \eq{rem_3_bdd} 
and
%$\|   \Grad \Psi_0 \|^2_{L_2(\GO \cap \CV_{h %d/2
%})} $
%we have
\begin{eqnarray}
&& \| \Grad \Psi_0
%(\Bx)
\|^2_{L^2 (\GO \cap \CV%_{h %d/2
%}
)} \leq \mbox{const} ~  \Gve^8 \sum_{1 \leq j \leq N} \int_{\GO \cap \CV%_{h %d/2
%}
} \fr{|C^{(j)}|^2 d \Bx}{|\Bx - \BO^{(j)}|^8} \nonumber \\
&& \leq \mbox{const  } %\fr{
\Gve^8  %}{d^5} 
\sum_{1 \leq j \leq N} |C^{(j)}|^2 \leq \mbox{const} \fr{\Gve^8}{d^3} % 8} 
\|\Grad v%_f
\|^2_{L^2(\GO)}. \label{rem_4_bdd}
\end{eqnarray}
%which completes 
Combining \eq{rem_3_bdd}--\eq{rem_4_bdd} we complete the proof. $\Box$
%\end{proof}

\section{Illustrative example} \label{example}
  
Now, the asymptotic approximation derived in the previous section is applied to the case of a relatively simple geometry, where all the terms  in the formula \eq{introeq1a} can be written explicitly. 


\subsection{The case of a domain with a cloud of spherical voids}
\label{cloud_example}

Let $\GO_N$ be  a ball of a finite radius $R$, with the centre at the origin, containing $N$ spherical voids $F^{(j)}$ of radii $\rho_j$ with the centres at $\BO^{(j)}, j=1,\ldots, N,$ as shown in Fig. \ref{diagramcloud}.
\begin{figure}[htbp]
%\psfrag{1}{\!\!\!\!\!\!$\scriptsize{R}$}
%\psfrag{2}{\!\!\!$\scriptsize{x_3}$}
%\psfrag{3}{\!\!\!$\scriptsize{x_1}$}
%\psfrag{4}{$\scriptsize{\omega}$}
%\psfrag{5}{$\scriptsize{x_2}$}
%\psfrag{6}{$\scriptsize{0}$}
%\psfrag{7}{$\scriptsize{\gamma}$}
%\psfrag{8}{$\scriptsize{\Omega}$}
\centering
\includegraphics[width=0.495\textwidth]{cloud1pdf.pdf}
\caption{Example configuration of a sphere containing a cloud of spherical voids in a the cube $\omega$.}
\label{diagramcloud}
\end{figure}
The radii of the voids are assumed to be smaller than the %separation 
distance between nearest neighbours. %, and the number $N$ of voids is sufficiently large. 
%The function $f(\Bx)$ is chosen in such a way that 
We put $\phi\equiv 0$ and
\beq
f(\Bx) = \left\{ \begin{array}{cc}
6 %(|\Bx|^2-\rho^2) (7 |\Bx|^2 -3 \rho^2) 
& \mbox{ when }   |\Bx|< \rho, \\
0 & \mbox{ when }    \rho < |\Bx| < R.
\end{array} \right.
\eequ{ex0}
Here, it is assumed that $\rho+ b  < |\BO^{(j)}| < R - b, ~ 1 \leq j \leq N, $ where $\rho$ and $b$ are positive constants independent of $\Gve$ and $d$.   


The function $u_N$ is 
%defined as 
the solution of the mixed boundary value problem for the Poisson equation:
\begin{eqnarray}
&&\GD u_N(\Bx) + f(\Bx) = 0, ~~\mbox{when  } \Bx \in \GO_N, \label{ex1} \\
&& u_N(\Bx) = 0,   ~~\mbox{when  } |\Bx| = R, \label{ex2} \\
&& \fr{\prt u_N}{\prt n}(\Bx) = 0, ~~\mbox{when  } |\Bx - \BO^{(j)}| = \rho_j, ~j = 1,\ldots,N. \label{ex3} 
\end{eqnarray}

In this case, $u_N$ is approximated by \eq{introeq1a}, where the solution of the %limit 
Dirichlet problem in $\GO$ is given by
\begin{equation}
v%_f 
(\Bx) = \left\{ \begin{array}{cc} %(\rho^2- |\Bx|^2)^3 
\rho^2 (3 -2 \rho R^{-1})  - |\Bx|^2 & \mbox{ when }   |\Bx|< \rho, \\
2 \rho^3 (|\Bx|^{-1}- R^{-1}) & \mbox{ when }    \rho < |\Bx| < R.
\end{array} \right.
\eequ{ex4}
In turn, the dipole fields $\BCD^{(j)}$ and the dipole matrices $\BCQ^{(j)}$ have the form
\begin{eqnarray}
\BCD^{(j)}(\Bx) = - \rho_j^3 \fr{\Bx - \BO^{(j)}}{|\Bx - \BO^{(j)}|^3}, ~~\BCQ^{(j)} = - 2 \pi \rho_j^3 I_3, \label{ex5}
\end{eqnarray}
where $I_3$ is the $3\times 3$ identity matrix.

The regular part $H(\Bx, \By)$ of Green's function in the % limit 
domain $\GO$ (see \eq{H_def}) is 
\beq
H(\Bx, \By) = \fr{R}{4 \pi |\By| |\Bx - \hat{\By}|}, ~~ \hat{\By} = \fr{R^2}{|\By|^2} \By. 
\eequ{ex6}
The coefficients $\BC^{(j)}, ~j = 1, \ldots, N,$ in %the asymptotic formula 
\eq{introeq1a} are defined from the algebraic system
\eq{R3formalgeq9a}, where Green's function $G(\Bx, \By)$ is given by
\beq
G(\Bx, \By) = \fr{1}{4 \pi |\Bx - \By|} - \fr{R}{4 \pi |\By| |\Bx - \hat{\By}|}.
\eequ{ex7}

\subsection{Finite elements simulation versus the asymptotic approximation}
%\subsection*{Example 1: Mesoscale cloud of spherical voids}
The explicit representations of the fields $v, {\BCD}^{(j)}, H, G$, given above, are used in the asymptotic formula
\eq{introeq1a}. Here, we present a comparison between the results of an independent Finite Element computation, produced in COMSOL, and the mesoscale asymptotic approximation \eq{introeq1a}. 


 
%In our first example
For the computational example, we set $R=120$, and consider a cloud of $N=18$ spherical voids arranged into a cloud of a
parallelipiped shape. The  position of the centre and radius of each void is included in Table \ref{Table1a}. The support of the function $f$ (see (\ref{ex0})), is chosen to be inside the sphere with radius $\rho=30$ and  centre at the origin,
as stated in \eq{ex0}.  
\begin{table}[htbp]\centering
\label{tabincdata}
\begin{tabular}{|c|c|c||c|c|c|}
 \hline\hline Void & Centre & $\rho_j /R$ &  Void & Centre & $\rho_j/R$\\
\hline\hline $F^{(1)}$   &(-50, 0, 0)&  0.0417 &  $F^{(10)}$   &(-72, 0, 0)& 0.0417 \\
\hline $F^{(2)}$   &(-50, 0, 22)&  0.0333 &  $F^{(11)}$   &(-72, 0, 22) & 0.0458\\
\hline $F^{(3)}$   &(-50, 22, 0)&  0.0292&  $F^{(12)}$   &(-72, 22, 0) & 0.0292\\
\hline $F^{(4)}$   &(-50, 0, -22)& 0.0375  &  $F^{(13)}$   &(-72, 0, -22) &  0.0375    \\
\hline $F^{(5)}$   &(-50, -22, 0)& 0.0458   &  $F^{(14)}$   &(-72, -22, 0) & 0.0417 \\
\hline $F^{(6)}$   &(-50, 22, 22)& 0.0292  &  $F^{(15)}$   &(-72, 22, 22) & 0.0333\\
\hline $F^{(7)}$   &(-50, 22, -22)& 0.025  &  $F^{(16)}$   &(-72, 22, -22)& 0.05  \\
\hline $F^{(8)}$   &(-50, -22, 22)&  0.0375  &  $F^{(17)}$   &(-72, -22, 22)& 0.0333 \\
\hline $F^{(9)}$   &(-50, -22, -22)& 0.0375   &  $F^{(18)}$   &(-72, -22, -22)& 0.0375\\
\hline
\end{tabular}
\caption{Data for the voids $F^{(j)}$, $j=1, \dots, 18$.}
\label{Table1a}
\end{table}


Figure \ref{fig1} shows the asymptotic solution $u_N$ of the mixed boundary value problem (part (b) of the figure) and its numerical counterpart obtained in COMSOL 3.5 (part (a) of the figure). This computation  has been produced for a spherical body containing $18$ small voids defined in Table \ref{Table1a}. 
%In part (a), the colour map shows the function $u_N$ evaluated numerically in COMSOL 3.5, whereas part (b) presents the asymptotic approximation obtained according to the formula  \eq{introeq1a}. 
The relative error for the chosen configuration
does not exceed $2 \% ,$ which confirms a very good agreement between the asymptotic and numerical results, which are
visually indistinguishable in Fig. \ref{fig1}a and Fig. \ref{fig1}b.

%The comparison between the analytical numerical approximation and the results of independent numerical computations in COMSOL shows a very good agreement, and the results are illustrated in Fig. \ref{fig1}. 

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.5]{numpdf.pdf} ~~~~\includegraphics[scale=0.5]{asypdf.pdf}
\end{center}
\centerline{(a)   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~  (b)}
\caption{Perforated domain containing %many 
$18$ holes: (a) Numerical solutions produced in COMSOL; (b) Asymptotic approximation.} \label{fig1}
\end{figure}

The computation was performed on Apple Mac, with 4Gb of RAM, and the number $N=18$ was chosen because any further increase in the number of voids resulted in a large three-dimensional computation, which exceeded the amount of available memory.
Although, increase in RAM can allow for a larger computation, it is evident that  three-dimensional finite element computations for a mesoscale geometry have serious limitations. On the other hand, the analytical asymptotic formula can still be used on the same computer for sigtnificantly larger number of voids.

In the next subsection, we show such an example where the number of voids within the mesoscale cloud runs upto $N=1000$, which would simply be unachievable in a finite element computation in COMSOL 3.5 with the same amount of RAM available.

  


==> Mesoscale pdf/macroarx.tex <==
% Reduce space surrounding equal signs (=) in equation arrays.
\setlength{\arraycolsep}{2pt}
% Set up counter for list environments
\newcounter{itemnbr}
% Handy abbreviations.
\newcommand\eq[1] {(\ref{#1})}
\newcommand\eqp[1] {(\ref{eq:#1})}
%\newcommand\defn[1] {\ref{def:#1}}
%\newcommand\thm[1] {\ref{thm:#1}}
\newcommand\sect[1] {\ref{sec:#1}}
\newcommand\fig[1] {\ref{fig:#1}}
\newcommand\labeq[1] {\label{eq:#1}}
\newcommand\labdefn[1] {\label{def:#1}}
\newcommand\labthm[1] {\label{thm:#1}}
\newcommand\labsect[1] {\label{sec:#1}}
\newcommand\labfig[1] {\label{fig:#1}}
%\newcommand\etal{{\it et al.}}
%\newcommand\B {\Bigg}
%\newcommand\frak {\mathfrak}
% Math environments
%\newtheorem{definition}{Definition}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newcommand\proof{{\it Proof:}\quad}
%\newcommand\remark{{\it Remark:}\quad}
%\newcommand\qed{\ \rule[-0.2ex]{0.3em}{1.5ex}}
% De-verbose the LaTeX math environment
\newcommand{\bfm}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\nonum}{\nonumber \\}
\newcommand{\beqa}{\begin{eqnarray}}
%\newcommand{\eeqa}[1]{\label{#1}\end{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bequ}{\begin{equation}}
\newcommand{\eequ}[1]{\label{#1}\end{equation}}
%\newcommand{\R}{\mbox{R}}
%\newcommand{\C}{\mbox{C}}
\newcommand{\Grad}{\nabla}
%\newcommand{\Div}{\nabla \cdot}
\newcommand{\Curl}{\nabla \times}
\newcommand{\mn}{{\rm min}}
\newcommand{\mx}{{\rm max}}
\newcommand{\lang}{\langle}
\newcommand{\rang}{\rangle}
\newcommand{\Md}{\partial}
\newcommand{\MP}{\bigoplus}
\newcommand{\MT}{\bigotimes}
\newcommand{\MU}{\bigcup}
\newcommand{\MI}{\bigcap}
\newcommand{\MV}{\bigvee}
\newcommand{\MW}{\bigwedge}
\newcommand{\ov}[1]{\overline{#1}}

% Abbreviate definitions of greek symbols
\newcommand{\Ga}{\alpha}
\newcommand{\Gb}{\beta}
\newcommand{\Gd}{\delta}
\newcommand{\Ge}{\epsilon}
\newcommand{\Gve}{\varepsilon}
\newcommand{\Gf}{\phi}
\newcommand{\Gvf}{\varphi}
\newcommand{\Gg}{\gamma}
\newcommand{\Gc}{\chi}
\newcommand{\Gi}{\iota}
\newcommand{\Gk}{\kappa}
\newcommand{\Gl}{\lambda}
\newcommand{\Gn}{\eta}
\newcommand{\Gm}{\mu}
\newcommand{\Gv}{\nu}
\newcommand{\Gp}{\pi}
\newcommand{\Gt}{\theta}
\newcommand{\Gvt}{\vartheta}
\newcommand{\Gr}{\rho}
\newcommand{\Gvr}{\varrho}
\newcommand{\Gs}{\sigma}
\newcommand{\Gvs}{\varsigma}
\newcommand{\Gj}{\tau}
\newcommand{\Gu}{\upsilon}
\newcommand{\Go}{\omega}
\newcommand{\Gx}{\xi}
\newcommand{\Gy}{\psi}
\newcommand{\Gz}{\zeta}
\newcommand{\GD}{\Delta}
\newcommand{\GF}{\Phi}
%\newcommand{\GG}{\Gamma}
\newcommand{\GL}{\Lambda}
\newcommand{\GP}{\Pi}
\newcommand{\GT}{\Theta}
\newcommand{\GS}{\Sigma}
\newcommand{\GU}{\Upsilon}
\newcommand{\GO}{\Omega}
\newcommand{\GX}{\Xi}
\newcommand{\GY}{\Psi}

% Abbreviate definitions of bold greek symbols: note that defs.tex is
% needed first
\newcommand{\BGa}{\bfm\alpha}
\newcommand{\BGb}{\bfm\beta}
\newcommand{\BGd}{\bfm\delta}
\newcommand{\BGe}{\bfm\epsilon}
\newcommand{\BGve}{\bfm\varepsilon}
\newcommand{\BGf}{\bfm\phi}
\newcommand{\BGvf}{\bfm\varphi}
\newcommand{\BGg}{\bfm\gamma}
\newcommand{\BGc}{\bfm\chi}
\newcommand{\BGi}{\bfm\iota}
\newcommand{\BGk}{\bfm\kappa}
\newcommand{\BGl}{\bfm\lambda}
\newcommand{\BGn}{\bfm\eta}
\newcommand{\BGm}{\bfm\mu}
\newcommand{\BGv}{\bfm\nu}
\newcommand{\BGp}{\bfm\pi}
\newcommand{\BGt}{\bfm\theta}
\newcommand{\BGvt}{\bfm\vartheta}
\newcommand{\BGr}{\bfm\rho}
\newcommand{\BGvr}{\bfm\varrho}
\newcommand{\BGs}{\bfm\sigma}
\newcommand{\BGvs}{\bfm\varsigma}
\newcommand{\BGj}{\bfm\tau}
\newcommand{\BGu}{\bfm\upsilon}
\newcommand{\BGo}{\bfm\omega}
\newcommand{\BGx}{\bfm\xi}
\newcommand{\BMx}{\bfm\xi}
\newcommand{\BGy}{\bfm\psi}
\newcommand{\BGz}{\bfm\zeta}
\newcommand{\BGD}{\bfm\Delta}
\newcommand{\BGF}{\bfm\Phi}
\newcommand{\BGG}{\bfm\Gamma}
\newcommand{\BGL}{\bfm\Lambda}
\newcommand{\BGP}{\bfm\Pi}
\newcommand{\BGT}{\bfm\Theta}
\newcommand{\BGS}{\bfm\Sigma}
\newcommand{\BGU}{\bfm\Upsilon}
\newcommand{\BGO}{\bfm\Omega}
\newcommand{\BGX}{\bfm\Xi}
\newcommand{\BGY}{\bfm\Psi}


% Abbreviate symbols for caligraphic letters
\newcommand{\Ca}{{\cal a}}
\newcommand{\Cb}{{\cal b}}
\newcommand{\Cc}{{\cal c}}
\newcommand{\Cd}{{\cal d}}
\newcommand{\Ce}{{\cal e}}
\newcommand{\Cf}{{\cal f}}
\newcommand{\Cg}{{\cal g}}
\newcommand{\Ch}{{\cal h}}
\newcommand{\Ci}{{\cal i}}
\newcommand{\Cj}{{\cal j}}
\newcommand{\Ck}{{\cal k}}
\newcommand{\Cl}{{\cal l}}
\newcommand{\Cm}{{\cal m}}
\newcommand{\Cn}{{\cal n}}
\newcommand{\Co}{{\cal o}}
\newcommand{\Cp}{{\cal p}}
\newcommand{\Cq}{{\cal q}}
\newcommand{\Cr}{{\cal r}}
\newcommand{\Cs}{{\cal s}}
\newcommand{\Ct}{{\cal t}}
\newcommand{\Cu}{{\cal u}}
\newcommand{\Cv}{{\cal v}}
\newcommand{\Cx}{{\cal x}}
\newcommand{\Cy}{{\cal y}}
\newcommand{\Cz}{{\cal z}}
\newcommand{\CA}{{\cal A}}
\newcommand{\CB}{{\cal B}}
%\newcommand{\CC}{{\cal C}}
%\newcommand{\CD}{{\cal D}}
\newcommand{\CE}{{\cal E}}
\newcommand{\CF}{{\cal F}}
%\newcommand{\CG}{{\cal G}}
\newcommand{\CH}{{\cal H}}
\newcommand{\CI}{{\cal I}}
\newcommand{\CJ}{{\cal J}}
\newcommand{\CK}{{\cal K}}
\newcommand{\CL}{{\cal L}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CN}{{\cal N}}
\newcommand{\CO}{{\cal O}}
\newcommand{\CP}{{\cal P}}
\newcommand{\CQ}{{\cal Q}}
\newcommand{\CR}{{\cal R}}
\newcommand{\CS}{{\cal S}}
\newcommand{\CT}{{\cal T}}
\newcommand{\CU}{{\cal U}}
\newcommand{\CV}{{\cal V}}
\newcommand{\CW}{{\cal W}}
\newcommand{\CX}{{\cal X}}
\newcommand{\CY}{{\cal Y}}
\newcommand{\CZ}{{\cal Z}}
% Abbreviate symbols for bold caligraphic letters
\newcommand{\BCa}{{\bfm{\cal a}}}
\newcommand{\BCb}{{\bfm{\cal b}}}
\newcommand{\BCc}{{\bfm{\cal c}}}
\newcommand{\BCd}{{\bfm{\cal d}}}
\newcommand{\BCe}{{\bfm{\cal e}}}
\newcommand{\BCf}{{\bfm{\cal f}}}
\newcommand{\BCg}{{\bfm{\cal g}}}
\newcommand{\BCh}{{\bfm{\cal h}}}
\newcommand{\BCi}{{\bfm{\cal i}}}
\newcommand{\BCj}{{\bfm{\cal j}}}
\newcommand{\BCk}{{\bfm{\cal k}}}
\newcommand{\BCl}{{\bfm{\cal l}}}
\newcommand{\BCm}{{\bfm{\cal m}}}
\newcommand{\BCn}{{\bfm{\cal n}}}
\newcommand{\BCo}{{\bfm{\cal o}}}
\newcommand{\BCp}{{\bfm{\cal p}}}
\newcommand{\BCq}{{\bfm{\cal q}}}
\newcommand{\BCr}{{\bfm{\cal r}}}
\newcommand{\BCs}{{\bfm{\cal s}}}
\newcommand{\BCt}{{\bfm{\cal t}}}
\newcommand{\BCu}{{\bfm{\cal u}}}
\newcommand{\BCv}{{\bfm{\cal v}}}
\newcommand{\BCx}{{\bfm{\cal x}}}
\newcommand{\BCy}{{\bfm{\cal y}}}
\newcommand{\BCz}{{\bfm{\cal z}}}
\newcommand{\BCA}{{\bfm{\cal A}}}
\newcommand{\BCB}{{\bfm{\cal B}}}
\newcommand{\BCC}{{\bfm{\cal C}}}
\newcommand{\BCD}{{\bfm{\cal D}}}
\newcommand{\BCE}{{\bfm{\cal E}}}
\newcommand{\BCF}{{\bfm{\cal F}}}
\newcommand{\BCG}{{\bfm{\cal G}}}
\newcommand{\BCH}{{\bfm{\cal H}}}
\newcommand{\BCI}{{\bfm{\cal I}}}
\newcommand{\BCJ}{{\bfm{\cal J}}}
\newcommand{\BCK}{{\bfm{\cal K}}}
\newcommand{\BCL}{{\bfm{\cal L}}}
\newcommand{\BCM}{{\bfm{\cal M}}}
\newcommand{\BCN}{{\bfm{\cal N}}}
\newcommand{\BCO}{{\bfm{\cal O}}}
\newcommand{\BCP}{{\bfm{\cal P}}}
\newcommand{\BCQ}{{\bfm{\cal Q}}}
\newcommand{\BCR}{{\bfm{\cal R}}}
\newcommand{\BCS}{{\bfm{\cal S}}}
\newcommand{\BCT}{{\bfm{\cal T}}}
\newcommand{\BCU}{{\bfm{\cal U}}}
\newcommand{\BCV}{{\bfm{\cal V}}}
\newcommand{\BCW}{{\bfm{\cal W}}}
\newcommand{\BCX}{{\bfm{\cal X}}}
\newcommand{\BCY}{{\bfm{\cal Y}}}
\newcommand{\BCZ}{{\bfm{\cal Z}}}


\def\ii{{\rm i}}
\def\dd{{\rm d}}
\def\Im{{\it Im}}
\def\Re{{\it Re}}
\def\ca{{\cal A}}
\def\ct{{\cal T}}
\def\Ba{{\bf a}}
\def\Bb{{\bf b}}
\def\Bc{{\bf c}}
\def\Bd{{\bf d}}
\def\Be{{\bf e}}
\def\Bf{{\bf f}}
\def\Bg{{\bf g}}
\def\Bh{{\bf h}}
\def\Bi{{\bf i}}
\def\Bj{{\bf j}}
\def\Bk{{\bf k}}
\def\Bl{{\bf l}}
\def\Bm{{\bf m}}
\def\Bn{{\bf n}}
\def\Bo{{\bf o}}
\def\Bp{{\bf p}}
\def\Bq{{\bf q}}
\def\Br{{\bf r}}
\def\Bs{{\bf s}}
\def\Bt{{\bf t}}
\def\Bu{{\bf u}}
\def\Bv{{\bf v}}
\def\Bw{{\bf w}}
\def\Bx{{\bf x}}
\def\By{{\bf y}}
\def\Bz{{\bf z}}
\def\BA{{\bf A}}
\def\BB{{\bf B}}
\def\BC{{\bf C}}
\def\BD{{\bf D}}
\def\BE{{\bf E}}
\def\BF{{\bf F}}
\def\BG{{\bf G}}
\def\BH{{\bf H}}
\def\BI{{\bf I}}
\def\BJ{{\bf J}}
\def\BK{{\bf K}}
\def\BL{{\bf L}}
\def\BM{{\bf M}}
\def\BN{{\bf N}}
\def\BO{{\bf O}}
\def\BP{{\bf P}}
\def\BQ{{\bf Q}}
\def\BR{{\bf R}}
\def\BS{{\bf S}}
\def\BT{{\bf T}}
\def\BU{{\bf U}}
\def\BV{{\bf V}}
\def\BW{{\bf W}}
\def\BX{{\bf X}}
\def\BY{{\bf Y}}
\def\BZ{{\bf Z}}

\def\half{{\scriptstyle{1\over 2}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\overliner}{\begin{eqnarray}}
\newcommand{\earr}{\end{eqnarray}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
\newcommand{\overlinern}{\begin{eqnarray*}}
\newcommand{\earrn}{\end{eqnarray*}}
\newcommand{\prt}{\partial}
\newcommand{\sg}{\sigma}
\newcommand{\fr}{\frac}
\newcommand{\kap}{\varkappa}
%\newcommand{\diag}{\mbox{diag}}
\newcommand{\sign}{\mbox{sign}}
\def\l{\label}
